A Closer Look at Novel Class Discovery from the Labeled Set

Novel class discovery (NCD) aims to infer novel categories in an unlabeled dataset leveraging prior knowledge of a labeled set comprising disjoint but related classes. Existing research focuses primarily on utilizing the labeled set at the methodological level, with less emphasis on the analysis of the labeled set itself. Thus, in this paper, we rethink novel class discovery from the labeled set and focus on two core questions: (i) Given a specific unlabeled set, what kind of labeled set can best support novel class discovery? (ii) A fundamental premise of NCD is that the labeled set must be related to the unlabeled set, but how can we measure this relation? For (i), we propose and substantiate the hypothesis that NCD could benefit more from a labeled set with a large degree of semantic similarity to the unlabeled set. Specifically, we establish an extensive and large-scale benchmark with varying degrees of semantic similarity between labeled/unlabeled datasets on ImageNet by leveraging its hierarchical class structure. As a sharp contrast, the existing NCD benchmarks are developed based on labeled sets with different number of categories and images, and completely ignore the semantic relation. For (ii), we introduce a mathematical definition for quantifying the semantic similarity between labeled and unlabeled sets. In addition, we use this metric to confirm the validity of our proposed benchmark and demonstrate that it highly correlates with NCD performance. Furthermore, without quantitative analysis, previous works commonly believe that label information is always beneficial. However, counterintuitively, our experimental results show that using labels may lead to sub-optimal outcomes in low-similarity settings.

==> sections/00_abstract.tex <==
%%% version 1
% \begin{abstract}
%     \red{Outdated}
%     The goal of NCD is to infer novel object categories in an unlabeled set using knowledge from a 
%     labeled set consisting of different but correlated classes. 
%     Existing studies mostly focus on approaches of enhancing NCD performance while ignoring the fundamental reasons that impact NCD performance.
%     In our work, we first propose two hypotheses about the underlying causes that affect the performance of NCD: 
%     (1) Categorical discrepancy: the discrepancy among new classes in unlabeled set. 
%     (2) Domain discrepancy: the domain discrepancy between labeled data and unlabeled data.  
%     Previous works took a lot of effort on utilizing knowledge from the labeled domain to 
%     improve a general-purpose clustering model. 
%     They, however, neglect the fundamental question of whether the unlabeled domain is related to 
%     the labeled domain, and how to quantify their correlation. 
%     We verify these two hypotheses by conducting experiments using data settings with 
%     various semantic domain discrepancies. Furthermore, we innovate two measurement definitions 
%     for evaluating categorical and domain discrepancy quantitatively. Based on these two assumptions, 
%     we propose a method, through pulling the domain discrepancy and pushing the categorical discrepancy, 
%     which outperforms the state of the art on standard benchmarks.
% \end{abstract}

%% version 2
\begin{abstract}
Novel class discovery (NCD) is to infer novel categories in an unlabeled set using prior knowledge of a labeled set comprising diverse but related classes.
However, \emph{how labeled sets impact unlabeled sets is still unclear}.
In this paper, we first demonstrate that given an unlabeled set, the closer the relationship between the labeled set and the unlabeled set, the better the performance of the unlabeled set.
This correlation remains true across a variety of state-of-the-art methodologies and typical NCD datasets, according to our experiments.
Based on this, we propose 'Transfer Leakage', a mathematical metric on calculating the relation between labeled set and unlabeled set.
Furthermore, we provide the 'Distinct Difficulty Benchmarks' (DDB) based on large-scale ImageNet, which better respects the objective of identifying new categories with three different difficulty levels, when the prior only has one.
Secondly, we investigated how each labeled set component influences unlabeled sets, including the supervised pre-trained model and image (i.e., X) without labels.
Surprisingly, we discover that even if we do not use the labels from the labeled set, we can still obtain similar results across different approaches and datasets.
Based on this finding, we propose our method which only use X information, and we achieve ....

\end{abstract}


% 对于ncd来说，我们要探讨一个核心问题：
% labeled是怎样影响unlabeled performance？

% 一个假设：labeled set 相当于unlabeld set越接近 high level senmantic，能为unlabeled sets提供越多信息。
% 基于这个假设，我们分别在cifar100和imagenet上得到验证，同时提供3 difficulty level benchmarks based on Imagenet.
% mathematically, we give a metric on measuring the how related between labeled set and unlabeled set.

% 共识：labels in labeled set 对 unlabeled set有帮助, 提供分类规则。
% 把标签拿到效果如何？我们得到了接近的结果。
% existing method 有很好的利用标签信息？
% label理论上在ncd有多大用？
% label到底有多大作用？ super-class label
% 除此之外，我们进一步探讨，labeled set 各 components对unlabeled
% set 的影响，我们分别探讨了supervised pre trained model，images, labels。
% 我们有两个发现： 1.pre trained model的影响不大； 2.即使我们仅使用X without Y, 我们仍能获得相对较好的效果。




==> sections/01_introduction.tex <==
\section{Introduction}
\label{sec:intro}
%%% 大背景
% NCD problem was initially described in \cite{han2019learning}
%%%% ncd: aim to discovering novel categories （NCD） from unlabeled sets by leveraging knowledge from labeled sets, which contain related and disjoint classes.
% 现今对于NCD的研究绝大部分都停留在方法层面上，都聚集在怎样更好地利用labeled 信息。DTC,RS通过 supervised pre-trained step to transfer the representation capability from the labeled set to the unlabeled set.
% openmix 通过mix up labeled and unlabeled sample 融合labeled 和unlabeled的信息，
% 还有利用self-supervised framework 把labeled和unlabeled同时加入训练，
% NCL ...
%而没有探究NCD的底层问题，比如说Label到底是怎样影响unlabeled，transfer给unlabel的“dark knowledge”到底是什么呢？
% "Meta": .... share high semantic feature
The combination of data, algorithms, and computer power has resulted in a boom in the field of artificial intelligence, particularly supervised learning with its large number of powerful deep models.
While these deep models are capable of properly identifying and clustering classes that are present in the training set (i.e., known/seen classes), they lack reliable extrapolation capacity when confronted with novel classes (i.e., unseen classes).
A classic illustration is how effortlessly a person can readily discriminate (cluster) unseen but similar vehicles (e.g., trains and steamships) based on prior experience.
This fact motivated researchers to develop a challenge termed novel class discovery (NCD)~\cite{han2019learning, chi2021meta, han2021autonovel, zhong2021neighborhood}, with the goal of discovering novel classes in an unlabeled dataset by leveraging knowledge from a labeled set, which contains related and disjoint classes.

% The NCD problem was initially described in \cite{han2019learning} with the goal of discovering novel classes in unlabeled set by leveraging knowledge from labeled sets, which contain related and disjoint classes.
Currently, the majority of research on NCD is at the methodological level, focusing on how to better utilize labeled information (e.g.,  in deep transfer clustering) while neglecting to explore the core problems in NCD from the ground root, with only one research \cite{chi2021meta} studying the NCD's solvability and indicating that NCD can be theoretically solved when labeled and unlabeled data share high-semantic feature.
%
However, many of the underlying issues of NCD remain a mystery, which constrains its development.
For example, (i) Given a specific unlabeled set,  \textit{what kind of labeled set can give the most benefit to it?}
(ii) An essential premise of NCD is that the labeled set should be related to the unlabeled set, but \textit{how can we measure this relation?}
(iii) There is a common belief in existing research: supervised knowledge from the labeled set is beneficial for discovering unknown classes. 
However, is this consensus always true? 
In other words, \textit{is supervised knowledge always beneficial for NCD problems?} 
And, how useful is the supervised knowledge? Is it possible that in some cases, supervised knowledge will not bring gain but loss?
% \begin{itemize}
%     \item Given a specific unlabeled set,  what kind of labeled set can give the most benefit to it?
%     \item The premise of NCD is labeled similar to unlabeled, can we measure the similarity?
%     \item There is a consensus in NCD: supervised knowledge benefit，if similarity is not very high, is supervised knowledge still useful?
% \end{itemize}

% 而忽略了对NCD的本质探究，仅有一篇文章focus on ..
% 但是，ncd 的很多底层问题仍然是谜团，这样的话束缚ncd的发展。
% Therefore, in this paper, we focus on ncd的三个本质问题。
% \begin{itemize}
%     \item Given a specific unlabeled set,  what kind of labeled set can give the most benefit to it?
%     \item The premise of NCD is labeled similar to unlabeled, can we measure the similarity?
%     \item There is a consensus in NCD: supervised knowledge benefit，if similarity is not very high, is supervised knowledge still useful?
% \end{itemize}


% 本文将探索下面三个问题：
% 1. 给定unlabeled set，怎样的labeled set能发挥更大的作用？
% 2. NCD 成立的前提是labeled related to unlabeled, 同时meta也指出, ncd theorically solved is that labeled and unlabeled share high-semantic feature, 但是这个related, high-semantic feature 应该怎么度量.或者说，how related can be regraded as related, labeled和unlabeled语义有多接近can be seen as share high-semantic feature
% 3. consensus：supervised knowledge benefit. 我们基于这个，提出一个疑问， 假如similarity 不是很高的情况下，supervised knowledge是不是依然有用？
% meta里面也指出，might not be necessary to introduce known-class data to help cluster novel-class data if known classes
% and novel classes do not share high-level semantic features.
% but，假设我们把supervised信息去掉，只剩下image信息呢？只用image信息能不能提高ncd性能
% “Due to the difference of inner-task, if we randomly sample data to compose an inner-task like existing
% meta-learning methods, these data may negatively influence each other in the training procedure. This
% is because these randomly sampled data in an inner-task have different clustering rules (Figure 3).”

For the first question, intuitively, we assume that higher semantic similarity labeled sets can provide more beneficial knowledge. 
We first verify our assumption on pairs of labeled and unlabeled sets, with varying semantic similarity between the labeled and the unlabeled set. This verification is performed on multiple NCD methods.
Existing benchmarks are insufficient for this because they only consider one labeled and unlabeled setinclude a single difficulty level.
Thus, we establish benchmarks with multiple levels of difficulty so that future research can test at multiple levels of difficulty.
Specifically, we make a new benchmark based on a large scale dataset, ImageNet \cite{deng2009imagenet} by leveraging its hierarchical semantic information.
It includes three difficulty levels, high-semantic similarity (easy), middle-semantic similarity (middle) and low-semantic similarity (hard), more detail in \ref{}.



% For the first question, intuitively, high semantic labeled set can provide more beneficial knowledge. 
% 基于这个假设， 我们首先在cifar100上基于语义相似性，划分不同相似性的（labele, unlabeled） pair.
% Empirically, we found that 对于同一个unlabeled set, high-semantic similarity labeled can 带来更多的提升 
% 基于这个，我们有理由质疑现有的benchmark是不完善的，我们应该设置不同难度的benchmark，以方便后续的研究在不同档位难度做测试 （ref openset）
    %  deleted 我们首先在split labeled and unlabeled set based on different level semantic similarity on cifar100, and verify our assumption on it.
    % 同时，我们认为现今对于ncd的研究在这方面是不完善，similarity level不同，最优的方法也可能不一样。
    % In other word, 对于不同similarity档位，优化的方法可能不一样。
    % 而现在的benchmark都只有一个similarity 档位，这显然不足而验证方法的有效性以及可行性。
% 因此，我们在imagenet的基础下make a new benchmark, including three different semantic similarity, high semantic，middle semantic and low semantic，分别对应easy，middle，hard 三个不同难度的档位。

% Secondly， ncd的motivation是利用related and different labeled set.... （前提）
% different 意思是类别不同，准确来说，应该是同一层级划分下，不同类别。
% 在fine-grained 下面，e.g., 牧羊犬 和腊肠犬属于不同类别；
% 但是coarse下，牧羊犬和腊肠犬都属于狗，和bird属于不同类别。
% 相对而言，different比related较容易定义，但是related应该怎么定义ne？
% meta， 。。。。多related can  be regarded as related, 有没有办法度量这个relation or similarity
% 基于这个疑问，we propose 一个新的度量semantic相似性的definition 基于maxium mean discrepancy.
% 具体来说，我们考虑一个情景，假如已获得trained labeled model，我们把unlabeled set feed into labeled model, 如果trained model 还能很好地classify unlabeled set，这意味着classify knowledge between labeled set and unlabeled set can be shared.
% In other word, labeled and unlabeled share high-semantic feature.
% 我们基于这个share feature 空间度量 semantic similarity  between l and u.

Secondly, an essential premise of NCD is that leveraging disjoint but related labeled set's information.
Additionally, \cite{chi2021meta} points out that the NCD is theoretically solved when labeled and unlabeled share high semantic feature.
Nevertheless, how related can be regrades as related?
Can we measure the relation?
Can we measure the extent of ``share high semantic feature''?
Further, the difficultly of our proposed benchmark also need to be measure.
Motivated by these, we propose a semantic similarity metric, defined as ``\textit{transfer leakage}".
Specifically, \textit{transfer leakage} quantifies the discriminative information in the labeled set leaked in the unlabeled set, that is, how much information we can leverage from the labeled dataset to help improve the performance of the unlabeled dataset, more detail in \ref{}.


% Thirdly, it is commonly believed that the supervised privileged knowledge is beneficial for NCD.
% 而我们的empirical 实验得出的结论有所不同。
% 我们分别在state-of-the-art uno 以及 typical rs上进行验证on cifar100, and our benchmark which build on imagenet.
% 我们做了三个对比实验：
% 1）only use unlabeled set
% 2) unlabeled set and labeled set's image 
% 3) unlabeled set and labeled set
% finding:
% 1.labeled set's image always helpful
% 2. supervised knowledge 在high semantic下有作用，然而在low semantic下，甚至有可能导致更worse的效果。
% 基于这个worse的效果，我们做进一步研究，supervised到底提供的是什么信息?
% 我们认为是rule规则，如果分类不一致，效果会变差，。。。。

Thirdly, it is commonly believed that the supervised privileged knowledge is beneficial for discovering unknown categories.
Does this hold true in any NCD settings, and if so, how significant is supervised knowledge?
According to the above hypothesis, we conduct the comparison experiments under the following data settings on CIFAR100 and our benchmark:
(i) only the unlabeled set without the labeled set
(ii) the unlabeled set and the labeled set's image without labeles;
(iii) the unlabeled set and the labeled set's image with labeles;
% Based on the consensus, it is expect that (iii) would performs much better than (ii).
% However, we can easily find counter results: on low-semantic similarity benchmark, the settings without labels even perform better than 



% In this work, we examine such a common belief through 


% The NCD problem was initially described in \cite{han2019learning}. During training, data are separated into labeled and unlabeled sets with the assumption that classes are related but distinct.
% The motivation in NCD is that discovering novel classes in unlabeled set by leveraging prior related labeled set's knowledge.
% Furthermore, \cite{chi2021meta} points out that NCD can be theorically solved when labeled and unlabeled share high-semantic feature.
% %%% first question
% However, how can high-semantic features be defined?
% And how closely between labeled sets and unlabeled sets can be generally considered related?
% Can we measure the semantic similarity between labeled and unlabeled?
% %%%%First contribution
% Inspired by these, we propose a similarity metric, named 'transfer leakage'.
% Intuitively, higher semantic similarity can provide more knowledge.
% We first verify this assumption on different semantic level data settings and measure the similarity based on transfer leakage.
% We confirm the reliability of transfer leakage.

% %%%%% second questions
% There is a consensus in NCD: supervised knowledge can benefit for discover  unknown classes.
% We suspect
% %%%%%second contribution:






% and has since inspired a rich line of research\cite{han2020automatically,han2021autonovel,zhong2021openmix,fini2021unified,zhong2021neighborhood,zhao2021novel},

% The NCD problem was initially formalized in \cite{han2019learning} and has since inspired a rich line of research\cite{han2020automatically,han2021autonovel,zhong2021openmix,fini2021unified,zhong2021neighborhood,zhao2021novel}, which focus on proposing a more efficient method of leveraging labeled sets' supervised information.
% \cite{chi2021meta} points out that NCD can be theoretically solved when known classes and novel classes share high-level semantic features.

% Generally, NCD is on the basic of labeled and unlabeled classes have related semantic similarity.

% All these methods are based on the consensus that `` the supervised knowledge from labeled sets are helpful for discovering unknown classes in unlabeled sets. "

% 1. How labeled set help unlabeled set？
% 2. consensus: network can benefit from the supervision available on the labeled set to learn rich image representations that can be transferred to discover unknown classes in the unlabeled set.

We summarise our contributions as follows:
\begin{itemize}
    \vspace{-0.1cm}
    \item We propose a metric for measuring the semantic similarity between labeled and unlabeled.
    \vspace{-0.1cm}
    \item Supervised knowledge may not benefit for NCD.
    \vspace{-0.1cm}
    \item We propose a three difficulty level benchmark for NCD.
\end{itemize}

%%NCD是建立在labeled set helpful for unlabeled set to discover novel class; However, 目前的研究大部分都在方法上用力，而没有探索labeled set是怎样提高unlabeled performance，（怎样帮助）why it can help？what’s the dark knowledge？
% 
% 我们首先从两个问题出发，
% 1.怎样的labeled set能为unlabeledset提供helpful knowledge?; 基于这点，我们提出一个猜想，higher semantic similarity ，more helpful knowledge
% 2. supervised information really help？
%质疑： 

% %% 背景
% %% version 1
% The requirement for large annotated training sets for deep learning is frequently a stumbling block. 
% For example, training a classification model necessitates a huge quantity of labeled data for each of the classes of interest and gathering adequate training data is costly or difficult, especially in medical areas.
% Also, we may come across novel categories that have never been annotated before and it's impossible to annotate all possible classes in some scenarios.
% Thus, we hope models can automatically discovery new categories among these data and leverage its potential information to improve model performance.

% Novel Class Discovery (NCD) has lately emerged as a viable solution to these difficulties. The goal of NCD is to train a network that can categorize a set of known classes while concurrently finding new ones in an unlabeled picture collection. The main idea for this setup is that the network would use the supervised information from labeled set to learn rich visual representations that can then be transferred to the unlabeled set to find new unknown classes.

% % 提出问题
% Existing work is focused on methods to improve the performance of NCD, while neglecting to investigate the underlying causes that affect NCD's performance.
% ~\cite{KaiHan2019LearningTD} first proposed NCD...
% ~\cite{fini2021unified} proposed a unified objective.
% And all existing works are following the same training setting as~\cite{KaiHan2019LearningTD}.

% We start from a thinking ``what 's the underlying causes to NCD's performance?".
% Then, we propose two assumptions: (1) Internal reason: the difficulty of doing clustering only on unlabeled data. (2) External reason: the domain gap between labeled data domain and unlabeled data domain.
% Firstly, if we first ignore labeled data, NCD would degraded to clustering problem. Thus, the difficulty of NCD lies only in the difficulty of doing clustering on unlabeled data.
% For the external reason, in NCD, there is a prerequisite assumption: the novel classes from unlabeled set should be different but related to labeled categories.  
% Intuitively, how related between labeled set and unlabeled set would impact NCD's performance directly.
% In other words, if the domain gap is smaller, more helpful knowledge would be provided for the unlabeled domain.
% We first verify these two assumptions under different data settings, and propose two measurements to quantify them i.e., self leakage and transfer leakage.

% Based on the two assumptions, we propose a new state-of-the-art method. 
% Specially, for the external reason, we pull the domain gap between labeled data and unlabeled data to transfer more helpful information for unlabeled set to find novel categories.
% For the internal reason, we push the domain gap between novel classes in unlabeled data to make data more distinguishable.

% \red{from meta,With the development of high-performance computing, we can train deep networks to achieve various tasks well (Deng et al., 2009; Song et al., 2019; Jing et al., 2020; Song et al., 2020; Liu et al., 2020b). However, the trained networks can only recognize the classes seen in the training set (i.e., known/seen classes), and cannot identify and cluster novel classes (i.e., unseen classes) like human beings. A prime example is that human can easily tell a novel animal category (e.g., okapi) after learning a few seen animal categories (e.g., horse and dog). Namely, human can effortlessly discover (cluster) novel categories of animals. Inspired by this fact, previous works formulated a novel problem called learning to discover novel classes (L2DNC) (Hsu et al., 2018; Han et al., 2019), where we train a clustering model using plenty of unlabeled novel-class and labeled known-class data.
% known classes and novel classes share high-level semantic features.
% This theorem shows that it might not be necessary to introduce known-class data to help cluster novel-class data if known classes and novel classes do not share high-level semantic features. Namely, L2DNC might be an ill-defined problem if known and novel class do not share high-level semantic features.}


% %% version 2
% The requirement for large annotated training sets for deep learning is frequently a stumbling block. 
% For example, training a classification model necessitates a huge quantity of labeled data for each of the classes of interest and gathering adequate training data is costly or difficult, especially in medical areas.
% Also, we may come across novel categories that have never been annotated before and it's impossible to annotate all possible classes in some scenarios.
% Thus, we hope models can automatically discovery new categories among these data and leverage its potential information to improve model performance.

% Novel Class Discovery (NCD) has lately emerged as a viable solution to these difficulties. The goal of NCD is to train a network that can categorize a set of known classes while concurrently finding new ones in an unlabeled picture collection. The main idea for this setup is that the network would use the supervised information from labeled set to learn rich visual representations that can then be transferred to the unlabeled set to find new unknown classes.

% % 提出问题
% Existing work is focused on methods to improve the performance of NCD, while neglecting to investigate the underlying causes that affect NCD's performance.
% ~\cite{han2019learning} first proposed NCD...
% ~\cite{fini2021unified} proposed a unified objective.
% And all existing works are following the same training setting as~\cite{han2019learning}.

% We start from a thinking ``what 's the underlying causes to NCD's performance?".
% Then, we propose two assumptions: (1) Internal reason: the difficulty of doing clustering only on unlabeled data. (2) External reason: the domain gap between labeled data domain and unlabeled data domain.
% Firstly, if we first ignore labeled data, NCD would degraded to clustering problem. Thus, the difficulty of NCD lies only in the difficulty of doing clustering on unlabeled data.
% For the external reason, in NCD, there is a prerequisite assumption: the novel classes from unlabeled set should be different but related to labeled categories.  
% Intuitively, how related between labeled set and unlabeled set would impact NCD's performance directly.
% In other words, if the domain gap is smaller, more helpful knowledge would be provided for the unlabeled domain.
% We first verify these two assumptions under different data settings, and propose two measurements to quantify them i.e., self leakage and transfer leakage.

% Based on the two assumptions, we propose a new state-of-the-art method. 
% Specially, for the external reason, we pull the domain gap between labeled data and unlabeled data to transfer more helpful information for unlabeled set to find novel categories.
% For the internal reason, we push the domain gap between novel classes in unlabeled data to make data more distinguishable.


==> sections/02_related_work.tex <==
\section{Related work and Preliminary}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \begin{table}[]
% \label{comparedtable}
% \begin{tabular}{@{}lccc@{}}
% \toprule
%         & NCD & SLL & TL  \\ \midrule
% Has $C_{u}$? & No  & No  & Yes \\
% $C_{u}=C_{l}$?  & No  & Yes & No  \\
% \bottomrule
% \end{tabular}
% \end{table}
% We summary the comparisons to semi-supervised learning (SSL), transfer learning and clustering in Fig. ~\ref{fig:compare}.\\

% \textbf{Novelty class discovery} 
\textbf{Related works.}
Novel class discovery (NCD) is a relatively new problem proposed in recent years, aiming to discover novel classes (i.e., assign them to several clusters) by making use of similar but different known classes.
Compared with unsupervised learning (Barlow, 1989), NCD also requires labeled known-class data to help cluster novel-class data. 
NCD is first formalized in DTC \cite{han2019learning}, but the study of NCD can be dated back to works, KCL \cite{hsu2018learning} and MCL \cite{hsu2019multi}.
Both of which maintain two models trained with labelled data and unlabelled data respectively, for general task transfer learning.

In DTC, they first learn a data embedding with metric learning on labeled data, then to employ the deep embedded clustering method \cite{han2019learning} to cluster the novel-class data.
Then, OpenMix \cite{zhong2021openmix} is proposed to mix known-class and novel-class data to learn a joint label distribution, benefiting to find their finer relations.
Both RS \cite{han2021autonovel,han2020automatically} and \cite{han2019learning} yield the pairwise similarity and use self-supervised learning to boost feature extraction while \cite{han2019learning} focused on local and global information, and used mutual knowledge distillation to promote information exchange and agreement.
NCL \cite{zhao2021novel} extracts and aggregates the pairwise pseudo-labels for the unlabelled data with contrastive learning and generates hard negatives by mixing the labelled and unlabelled data in the feature space.
UNO \cite{fini2021unified} combinates pseudo-labels with ground-truth labels in a unified objective function that enabled better cooperation and less interference without self-supervised learning.
In \cite{chi2021meta}, they find that NCD can be theoretical addressed when known and unknown classes are shared high-level semantic features, and propose a solution that link NCD to meta-learning.
% Chi et al. (2022) formulated NCD with a sampling
% process. They argued that the novel classes and known
% classes should have the same high-level semantic meanings. Based on this assumption, they proved that NCD can be
% theoretical addressed and linked NCD to meta-learning that served as the solution in their paper.




% \red{from GCD} The problem of novel category discovery (NCD) is formalized in DTC [17]. Earlier meth- ods that can be applied to this problem are KCL [19] and MCL [20], both of which maintain two models trained with labelled data and unlabelled data respectively, for general task transfer learning. AutoNovel (aka Rankstats) [15, 16] tackles the NCD problem with a three stage method. The model is firstly trained with self-supervision on all data for low-level representation learning. 
% Then, it is further trained with full supervision on labelled data to capture higher level semantic information. Finally, a joint learning stage is car- ried out to transfer knowledge from the labelled to unla- belled data with ranking statistics. Zhao and Han [48] pro- pose a model with two branches, one for global feature learning and the other for local feature learning, such that dual ranking statistics and mutual learning are conducted with these two branches for better representation learning and new class discovery. OpenMix [50] mixes the labelled and unlabelled data to avoid the model from over-fitting for NCD. NCL [49] extracts and aggregates the pairwise pseudo-labels for the unlabelled data with contrastive learn- ing and generates hard negatives by mixing the labelled and unlabelled data in the feature space for NCD. Jia et al. [21] propose an end-to-end NCD method for single- and multi-modal data with contrastive learning and winner- takes-all hashing. A unified cross-entropy loss is introduced in UNO [12] to allow the model to be trained on labelled and unlabelled data jointly by swapping the pseudo-labels from labelled and unlabelled classification heads.

% \red{from 2986} Novel class discovery is a relatively new problem proposed in recent years, aiming to discover novel classes (i.e., assign them to several clusters) by making use of similar but differ- ent known classes. The first two works that proposed NCD and tried to solve it were KL-Divergence-based contrastive loss (KCL) (Hsu et al., 2018) and meta classification likeli- hood (Hsu et al., 2019), which employed feature extractors to predict pairwise similarity of each novel-class data pair.
% Then, Han et al. (2019) proposed a deep transfer clustering (DTC) to first learn a data embedding with metric learning on labeled data, then to employ the deep embedded cluster- ing method (Xie et al., 2016) to cluster the novel-class data. 
% To further extract the information from the data embedding, Han et al. (2020; 2021) proposed to use the ranking statistics (RS) to yield the pairwise similarity and use self-supervised learning to boost feature extraction.

% Recently, OpenMix (Zhong et al., 2021b) is proposed to mix known-class and novel-class data to learn a joint label distribution, benefiting to find their finer relations. 


% Zhong et al.(2021a) then proposed a neighborhood contrastive learning (NCL) to generate better discriminative representations.
% Fini et al. (2021) used pseudo-labels in combination with ground-truth labels in a UNified Objective function (UNO) that enabled better cooperation and less interference without self-supervised learning. 

% Zhao & Han (2021) proposed a two branch method focused on local and global information, and used mutual knowledge distillation to promote information exchange and agreement.

% Although the above studies have proposed several algo-
% 122 rithms to address the NCD problem, the underlying assump-tion of NCD was unclear. To demystify the assumption of NCD, Chi et al. (2022) formulated NCD with a sampling
% process. They argued that the novel classes and known
% classes should have the same high-level semantic meanings. Based on this assumption, they proved that NCD can be
% theoretical addressed and linked NCD to meta-learning that served as the solution in their paper.



% \begin{figure}
% \centering
% \includegraphics[height=6.5cm]{figures/comparison.png}
% \caption{Comparison to semi-supervised learning and transfer learning.
% In semi-supervised learning, both labeled samples and unlabeled samples share the same categories while in NCD, the unlabeled set's categories are different to the labeled set's. Compared to transfer learning, target set is unlabeled in NCD.}
% \label{fig:compare}
% \end{figure}


% (Fig.~\ref{fig:example} shows an example).
% The distance between text and figure should be about 8~mm, the
% distance between figure and caption about 5~mm.
% \begin{figure}
% \centering
% \includegraphics[height=6.5cm]{eijkel2}
% \caption{One kernel at $x_s$ ({\it dotted kernel}) or two kernels at
% $x_i$ and $x_j$ ({\it left and right}) lead to the same summed estimate
% at $x_s$. This shows a figure consisting of different types of
% lines. Elements of the figure described in the caption should be set in
% italics,
% in parentheses, as shown in this sample caption. The last
% sentence of a figure caption should generally end without a full stop}
% \label{example}
% \end{figure}

\textbf{Background and preliminary.}
We first introduce a formal framework of NCD. 
$(\mb{X}^l, Y^l)$ and $(\mb{X}^u, Y^u)$ denote random samples under the \emph{labeled/unlabeled probability measures} $\mathbb{P}^l$ and $\mathbb{P}^u$, respectively.
Here $\mb{X}^l \in \mathcal{X}^l \subset \mathbb{R}^d$ and $\mb{X}^u \in \mathcal{X}^u \subset \mathbb{R}^d$ are the labeled/unlabeled feature vectors. $Y^l \in \mathcal{C}^l$ and $Y^u \in \mathcal{C}^u$ are the labels of labeled/unlabeled data, where $\mathcal{C}^l / \mathcal{C}^u$ is the label set under the labeled probability measure $\mathbb{P}^l / \mathbb{P}^u$.
There are labeled dataset $\mathcal{L}_n = (\mb{X}_i^{l}, Y_i^{l})_{i=1, \cdots, n}$ independently drawn from the labeled probability measure $\mathbb{P}^{l}$, and unlabeled dataset $ \mathcal{U}_m = (\mb{X}_i^{u})_{i=1, \cdot, m}$ independently drawn from the unlabeled probability measure $\mathbb{P}_{\mb{X}}^u$. \textbf{Our primary goal is to make prediction to $Y^u_i$ under the probability measure $\mathbb{P}^{u}$ given $\mb{X}_i^{u}$.} We now give a general definition of NCD.

\begin{definition}[Novel class discovery]
	Given a labeled probability measure $\mathbb{P}^l$ on $\mathcal{X}^l \times \mathcal{C}^l$, an unlabeled probability measure $\mathbb{P}^u$ on $\mathcal{X}^u \times \mathcal{C}^u$, and a labeled dataset $\mathcal{L}_n$ and an unlabeled dataset $\mathcal{U}_m$, novel class discovery aims to predict the labels of the unlabeled dataset based on $\mathcal{L}_n$ and $\mathcal{U}_m$, where $\mathcal{C}^u \neq \mathcal{C}^l$.
\end{definition}

% \sout{In general, NCD is a subgroup of transfer learning, with both domains and tasks are different. Yet, it has own distinct characteristics in the existence of new classes on the unlabeled dataset.} In Figure \ref{fig:compare}, we summarize the relationship/different among three major learning paradigms (with both labeled and unlabeled datasets): NCD, semi-supervised learning and transfer learning.

% Then, the training samples $\mathcal{D}_\old = (\mb{X}_{\old,i}, Y_{\old,i})^{n_\old}_{i=1}$ are independent and identically drawn from the old probability measure $\mathbb{P}_\old$ on $(\mb{X}_l, Y_l)$. Note that $\mathcal{C}^{(l)}$ may not be fully observed by $\mathcal{D}_\old$, thus we denote $\mathcal{C}^{\text{sub}}_{\old} = \text{set}\{ (Y_i)_{i=1}^n \}$ to clarify. 
% For the new distribution, we observe $n_\new$ independent and identically distributed unlabeled data $( \mb{X}_{\new, l})_{l=1}^m$. The new class with respect to the training sample $\mathcal{D}_\old$ is defined as $\mathcal{C}^u / \mathcal{C}^{\text{sub}}_{\old}$.

% \red{add more about the marginal information, and $\mathbb{P}_{Y|\mb{X}}$ only.}
% \subsection{Transfer leakage}
% Note that it is critical to measure the similarity between $\mathbb{P}^l$ and $\mathbb{P}^u$.
% % As indicated in Figure \ref{fig:compare}, NCD degenerates to the classical SSL when $\mathbb{P}^l = \mathbb{P}^u$, or the transductive transfer learning if $\mathbb{P}_{Y|\mb{X}}^l = \mathbb{P}_{Y|\mb{X}}^u$. 
% % \sout{Moreover, in practice, there are many pairs of labeled and unlabeled dataset to choose from. For example, fixing the unlabeled dataset as CIFAR-100, we can use CIFAR-10, CIFAR-50 or Image-NET as the labeled dataset. }
% Certainly, different pairs of labeled/unlabeled datasets yield various predictive performance. This leads to the core questions: 
% \begin{center}
% \vspace{-0cm}
% \textit{How much does the labeled dataset $\mathcal{L}_n$ under $\mathbb{P}^l$ can help to predict the label under $\mathbb{P}^u$?}
% \vspace{-0cm}
% \end{center}

% % \begin{itemize}
% % % 	\item How can we tell the self \textit{difficulty} of NCD under $\mathbb{P}^u$ based on unlabeled dataset $\mathcal{U}_m$?
% % 	\item How much does the labeled dataset $\mathcal{L}_n$ under $\mathbb{P}^l$ can help to predict the label under $\mathbb{P}^u$?
% % \end{itemize}
%  To address the questions, 
% %  we propose the concept of \textit{leakage} to measure the difficulty of NCD. Specifically, the first question concerns the self difficulty of NCD under an unsupervised manner, which predicts labels solely based on marginal information of $\mb{X}^{u}$, is highly related to the discriminative information leaked in the marginal distribution, namely \textit{self leakage}. For the second question, 
%  we introduce \textit{transfer leakage} to quantify the discriminative information in $\mathbb{P}^u$ leaked in $\mathbb{P}^l$, that is, how much information we can leverage from the labeled dataset to help improve the performance of the unlabeled dataset.

% % It is worth to point out that investigation of the questions not only can help us to construct benchmark dataset for fair numerical comparison of existing methods (see Section \red{???}), but also inspire our proposed method yielding state-of-the-art performance in NCD (see Section \red{???}).

% % \label{sec:preliminary}



% % \subsubsection{Overall leakage}
% % \red{Change to IPM to make it more general.}
% % To quantify the \emph{overall leakage} under the probability measure $\mathbb{P}^u$, we turn to measure the discrepancy of $\mb{X}^{u}$ given different labels $Y^u = c; (c \in \mathcal{C}^{u})$. For instance, given two labels $c, c' \in \mathcal{C}^u$, if there exists a transformation $h(\cdot)$ such that the distributions of $h(\mb{X}^u) | Y^u = c$ and $h(\mb{X}^u) | Y^u = c'$ are easily separable (or distance is large), then it is potential feasible to discriminate $c$ and $c'$ under an unsupervised manner. To this end, we introduce Maximum Mean Discrepancy (MMD; \citep{gretton2012kernel}) or Wasserstein-1 distance (\cite{pmlr-v70-arjovsky17a}) to quality the discrepancy of two distributions:
% % \begin{align}
% % 	\label{def:mmd}
% % 	\MMD_\mathcal{H} \big( \mathbb{P}^u_{\mb{X}^u | Y^u=c'}, \mathbb{P}^u_{\mb{X}^u | Y^u = c} \big) := \sup_{h \in \mathcal{H}} \Big( \mathbb{E}\big( h( \mb{X}^u) \mid Y^u = c \big) - \mathbb{E}\big( h( \mb{X}^u) \mid Y^u = c'\big) \Big)
% % \end{align}
% % where $\mathcal{H}$ is a class of functions $h: \mathcal{X}^u \to \mathbb{R}$, which is usually specified as the unit ball in a reproducing kernel Hilbert Space (RKHS), or a deep neural network as in W-GAN \citep{pmlr-v70-arjovsky17a}.
% % From \eqref{def:mmd}, when $\MMD$ is large, it provides a relatively large possibility to find a good transformation on $\mb{X}^u$ discriminating labels in an unsupervised manner. 

% % % \noindent \textbf{Remark.} In \eqref{def:mmd}, we use a generative model $\mathbb{Q}_{\mb{X}^u | Y^u=c}$ to quantify the overall leakage, one may suggest using a discriminative model $\mathbb{Q}( Y^u = c| \mb{X}^u ); (c \in \mathcal{C}^u)$ to quality the leakage of the prediction under $\mathbb{Q}$. It is sensible in supervised learning, when $(\mb{X}^u, Y^u)$ is observed in training set. In our case, our goal to measure the leakage based on an unsupervised manner, where the discrepancy of $\mathbb{Q}_{\mb{X}^u | Y^u=c}$ is more reasonable.

% % For multi-class discrepancy, we mimic the one-vs-rest nature by taking the minimum discrepancy over all rest classes, which takes the discrepancy to the closest class. Taken together, the overall leakage is defined as follows.
% % \begin{definition}[Self leakage]
% % 	\label{def:S-leak}
% % 	The self \textit{leakage} of NCD prediction on $\mathbb{P}^u$ is defined as 
% % 	\begin{equation}
% % 	\text{S-Leak}( \mathbb{P}^u ) = \mathbb{E} \Big( \MMD^2 \big( \mathbb{P}^u_{\mb{X}^u | Y^u }, \mathbb{P}^u_{\widetilde{\mb{X}}^u | \widetilde{Y}^u } \big) \Big),
% % 	\end{equation}
% % 	where $(\mb{X}^u, Y^u), (\widetilde{\mb{X}}^u, \widetilde{Y}^u) \sim \mathbb{P}^u$ are independent copies under $\mathbb{P}^u$, and the expectation is taken with respect to $Y^u$ and $\widetilde{Y}^u$. 
% % \end{definition}

% % \begin{lemma}
% % 	\label{lemma:ol-zero}
% % 	$\text{O-Leak}( \mathbb{P}^u ) = 0$ if and only if $Y^u$ is independent with $\mb{X}^u$, that is, for any $c \in \mathcal{C}^u$:
% % 	$$
% % 	\mathbb{P}^u( Y^u = c \mid \mb{X}^u ) = \mathbb{P}^u(Y^u = c).
% % 	$$
% % \end{lemma}
% % Lemma \ref{lemma:ol-zero} indicates that if there is no overall leakage on $\mb{X}^u$ when predicting $Y^u$, then the best way to predict $Y^u$ given $\mb{X}^u$ is majority voting on $Y^u$. In practice, NCD dataset are often pre-balanced, that is, $\mathbb{P}^u(Y^u = c) = 1/|\mathcal{C}^u|$ for all $c \in \mathcal{C}^u$. 
% % % Then, \eqref{eqn:ol_gen_model} can be replaced as $\mathbb{P}^u(Y^u=c|\mb{X}^u) = \mathbb{P}(Y^u = c' | \mb{X}^u)$, and the best prediction is random guess. 
% % Therefore, the proposed overall leakage is a reasonable criterion to measure the predictive information leakage on $\mb{X}^u$, and the overall difficulty of NCD.


% % Suppose the labels $(Y^u_i)_{i=1, \cdot, m}$ for the unlabeled dataset are observed, denote $\mathcal{U}_c = \{ \mb{X}^u_i \in \mathcal{U}_m: Y_i^u = c\}$ as the sub-sample set under label $c$, the \textit{overall leakage} is empirically evaluated as 
% % \begin{align}
% % 	\label{eqn:emp_overall_leak}
% % 	\widehat{\text{O-Leak}}( \mathbb{P}^u ) & = \frac{2}{m(m-1)} \sum_{1 \leq i < i' \leq m} \widehat{\MMD}^2_{\mathcal{H}} \big( \mathcal{U}_{Y_i^u}, \mathcal{U}_{Y^u_{i'}} \big) \\
% % 	& = \sum_{c, c' \in \mathcal{C}^u; c \neq c'} \frac{|\mathcal{U}_c||\mathcal{U}_{c'}|}{m(m-1)} \widehat{\MMD}^2_{\mathcal{H}} \big( \mathcal{U}_c, \mathcal{U}_{c'} \big),
% % \end{align}
% % where $\widehat{\MMD}_{\mathcal{H}}$ is an empirical evaluation of MMD based on $\mathcal{H}$. For example, 
% % letting $\mathcal{H} = \mathcal{H}_K$ as a RKHS, we have
% % \begin{align}
% % 	\label{eqn:emp_mmd}
% % 	\widehat{\MMD}^2_{\mathcal{H}} ( \mathcal{U}_{c}, \mathcal{U}_{c'}) & = \frac{1}{|\mathcal{U}_{c}| \big( |\mathcal{U}_{c}| - 1 \big)} \sum_{ \mb{X}, \mb{X}' \in \mathcal{U}_{c}; \mb{X} \neq \mb{X}'} k( \mb{X}, \mb{X}' ) \\
% % 	& + \frac{1}{|\mathcal{U}_{c'}| \big( |\mathcal{U}_{c'}| - 1 \big)} \sum_{ \mb{X}, \mb{X}' \in \mathcal{U}_{c'}; \mb{X} \neq \mb{X}'} k( \mb{X}, \mb{X}' ) \nonumber \\ 
% % 	& = \quad - \frac{1}{|\mathcal{U}_{c}| |\mathcal{U}_{c'}| } \sum_{ \mb{X} \in \mathcal{U}_{c} } \sum_{ \mb{X}' \in \mathcal{U}_{c'}} k( \mb{X}, \mb{X}'),
% % \end{align}
% % where $k(\cdot, \cdot)$ is a reproducing kernel, such as Gaussian kernel. Note that a large $\widehat{\text{O-Leak}}_m(\mathbb{P}^u )$ implies that there is clear discrepancy on $\mb{X}^u$ among different classes, which indicates potential capability of unsupervised learning with $\mb{X}^u$ predicting its label. In practice, $\mb{X}^u$ is usually replaced by a latent feature from representation learning.

% For unsupervised learning, it is usually quite difficult to learn such as good transformation solely based on $\mb{X}^u$. Instead, NCD takes account of the conditional probability $\mathbb{P}^l_{Y | \mb{X} }$ (usually presented by a pre-trained neural network) from a labeled dataset to help construct a transformation. Thus, we consider \emph{transfer leakage} of $\mathbb{P}^l$ on $\mathbb{P}^u$.

% The main idea is to quantify the discrepancy of $\mathbb{P}^l_{Y|\mb{X}}$ on $\mb{X}^u$ under the new measure $\mathbb{P}^u$. Then, \emph{transfer leakage} can be defined as follows.

% \begin{definition}[Transfer leakage]
% 	\label{def:T-leak}
% 	The transfer leakage of NCD prediction under $\mathbb{P}^u$ based on the labeled conditional probability $\mathbb{P}^l_{Y^l|\mb{X}^l}$ is 
% 	\begin{equation}
% 	\text{T-Leak}( \mathbb{P}^u, \mathbb{P}^l ) = \mathbb{E} \Big( \MMD^2 \big( \mathbb{P}^u_{ \mb{p}^l(\mb{X}) | Y }, \mathbb{P}^u_{\mb{p}^l(\mb{X}') \mid Y'} \big) \Big),
% 	\end{equation}
% 	where $(\mb{X}, Y), (\mb{X}', Y) \sim \mathbb{P}^u$ are independent copies, the expectation is taken with respect to $Y$ and $Y'$ under $\mathbb{P}^u$, and $\mb{p}^l(\mb{X}^u)$ is the conditional probability under $\mathbb{P}^l_{Y|\mb{X}}$ on an unlabeled instance $\mb{X}^u$, which is defined as
% 	$$
% 	\mb{p}^l(\mb{x}) = \big(\mathbb{P}^l\big( Y^l=c \mid \mb{X}^l = \mb{x} \big) \big)_{c \in \mathcal{C}^l}.
% 	$$
% \end{definition}
% With the similar manner in Definition \ref{def:O-leak}, the definition of transfer leakage is to measure the discrepancy of $\mb{p}(\mb{X}^u)$ under different new classes of $\mathbb{P}^u$, which indicates the  informative leakage of $\mathbb{P}^u$ on $\mathbb{P}^l$, and potential capability of transferring information from $\mathbb{P}^l$ to $\mathbb{P}^u$.

% \begin{lemma}
% 	\label{lemma:tl-zero}
% 	$\text{T-Leak}( \mathbb{P}^u, \mathbb{P}^l ) = 0$ if and only if $Y^u$ is independent with $\mb{p}^l(\mb{X}^u)$, that is, for any $c \in \mathcal{C}^u$:
% 	\begin{equation}
% 		\label{eqn:tl-indep}
% 		\mathbb{P}^u\big( Y^u = c \mid \mb{p}^l(\mb{X}^u) \big) = \mathbb{P}^u(Y^u = c).
% 	\end{equation}
% 	Moreover, if $ \mathbb{P}^u = \mathbb{P}^l$, then \eqref{eqn:tl-indep} can be replaced as:
% 	$$
% 	\mathbb{P}^l\big( Y^l = c \mid \mb{X}^l \big) = \mathbb{P}^l(Y^l = c).
% 	$$
% \end{lemma}

% Given an estimated conditional probability $\widehat{\mathbb{P}}^l_{Y^l|\mb{X}^l}$, usually presented as a pre-trained neural network, we evaluate $\mb{X}^u$ on $\widehat{\mathbb{P}}^l_{Y^l|\mb{X}^l}$ as $\widehat{\mb p}^l(\mb{X}^u) = \big(\widehat{\mathbb{P}}^l\big( Y^l=c | \mb{X}^l = \mb{X}^u \big) \big)_{c \in \mathcal{C}^u}$, then the empirical transfer leakage is computed as
% \begin{align}
% 	\label{eqn:emp_overall_leak}
% 	\widehat{\text{T-Leak}}( \mathbb{P}^u, \mathbb{P}^l ) & = \frac{2}{m(m-1)} \sum_{1\leq i< i' \leq m}  \widehat{\MMD}^2_{\mathcal{H}} \big( \widehat{\mb p}^l( \mathcal{U}_{Y_i^u} ),  \widehat{\mb p}^l( \mathcal{U}_{ Y^u_{i'} } ) \big) \nonumber \\
% 	& = \sum_{c, c' \in \mathcal{C}^u; c \neq c'} \frac{|\mathcal{U}_c| |\mathcal{U}_{c'}|}{m(m-1)} \widehat{\MMD}^2_{\mathcal{H}} \big( \widehat{\mb{p}}^l(\mathcal{U}_c), \widehat{\mb{p}}^l(\mathcal{U}_{c'}) \big),
% \end{align}
% where $\widehat{\mb p}^l( \mathcal{U}_c) = ( \widehat{\mb p}^l(\bm{X}^u), \mb{X}^u \in \mathcal{U}_c)$.

==> sections/03_first.tex <==
\section{How the whole labeled sets impact unlabeled sets' performance ?}
%\section{The correlation between labeled sets and unlabeled sets}
In this section, we first give definition of NCD, and then study the correlation between labeled sets and unlabeled set.
We verify that the closer the relationship between the labeled set and the unlabeled set, the better the performance of the unlabeled set across various approaches and datasets, including CIFAR100\cite{} and ImageNet \cite{} empirically.
Besides, we also propose a metric `transfer leakage' on calculating the how related between labeled sets and unlabeled sets.
Lastly, we provide the `Distinct Difficulty Benchmarks' (DDB) based on large-scale ImageNet, which better respects the objective of identifying new categories with three different difficulty levels, when the prior only has one.

% \subsection{Two Assumptions}


\subsection{Transfer leakage}
\label{lab:transfer leakage}
Note that it is critical to measure the similarity between $\mathbb{P}^l$ and $\mathbb{P}^u$.
Certainly, different pairs of labeled/unlabeled datasets yield various predictive performance. This leads to the core questions: 
\begin{center}
\vspace{-0cm}
\textit{How much does the labeled dataset $\mathcal{L}_n$ under $\mathbb{P}^l$ can help to predict the label under $\mathbb{P}^u$?}
\vspace{-0cm}
\end{center}


 To address the questions, we introduce \textit{transfer leakage} to quantify the discriminative information in $\mathbb{P}^u$ leaked in $\mathbb{P}^l$, that is, how much information we can leverage from the labeled dataset to help improve the performance of the unlabeled dataset.
For unsupervised learning, it is usually quite difficult to learn such as good transformation solely based on $\mb{X}^u$. Instead, NCD takes account of the conditional probability $\mathbb{P}^l_{Y | \mb{X} }$ (usually presented by a pre-trained neural network) from a labeled dataset to help construct a transformation. Thus, we consider \emph{transfer leakage} of $\mathbb{P}^l$ on $\mathbb{P}^u$.
The main idea is to quantify the discrepancy of $\mathbb{P}^l_{Y|\mb{X}}$ on $\mb{X}^u$ under the new measure $\mathbb{P}^u$. Then, \emph{transfer leakage} can be defined as follows.

\begin{definition}[Transfer leakage]
	\label{def:T-leak}
	The transfer leakage of NCD prediction under $\mathbb{P}^u$ based on the labeled conditional probability $\mathbb{P}^l_{Y^l|\mb{X}^l}$ is 
	\begin{equation}
	\text{T-Leak}( \mathbb{P}^u, \mathbb{P}^l ) = \mathbb{E} \Big( \MMD^2 \big( \mathbb{P}^u_{ \mb{p}^l(\mb{X}) | Y }, \mathbb{P}^u_{\mb{p}^l(\mb{X}') \mid Y'} \big) \Big),
	\end{equation}
	where $(\mb{X}, Y), (\mb{X}', Y) \sim \mathbb{P}^u$ are independent copies, the expectation is taken with respect to $Y$ and $Y'$ under $\mathbb{P}^u$, and $\mb{p}^l(\mb{X}^u)$ is the conditional probability under $\mathbb{P}^l_{Y|\mb{X}}$ on an unlabeled instance $\mb{X}^u$, which is defined as
	$$
	\mb{p}^l(\mb{x}) = \big(\mathbb{P}^l\big( Y^l=c \mid \mb{X}^l = \mb{x} \big) \big)_{c \in \mathcal{C}^l}.
	$$
	\red{need to brief introduce MMD}
\end{definition}
The definition of transfer leakage is to measure the discrepancy of $\mb{p}(\mb{X}^u)$ under different new classes of $\mathbb{P}^u$, which indicates the  informative leakage of $\mathbb{P}^u$ on $\mathbb{P}^l$, and potential capability of transferring information from $\mathbb{P}^l$ to $\mathbb{P}^u$.

\begin{lemma}
	\label{lemma:tl-zero}
	$\text{T-Leak}( \mathbb{P}^u, \mathbb{P}^l ) = 0$ if and only if $Y^u$ is independent with $\mb{p}^l(\mb{X}^u)$, that is, for any $c \in \mathcal{C}^u$:
	\begin{equation}
		\label{eqn:tl-indep}
		\mathbb{P}^u\big( Y^u = c \mid \mb{p}^l(\mb{X}^u) \big) = \mathbb{P}^u(Y^u = c).
	\end{equation}
	Moreover, if $ \mathbb{P}^u = \mathbb{P}^l$, then \eqref{eqn:tl-indep} can be replaced as:
	$$
	\mathbb{P}^l\big( Y^l = c \mid \mb{X}^l \big) = \mathbb{P}^l(Y^l = c).
	$$
\end{lemma}

Given an estimated conditional probability $\widehat{\mathbb{P}}^l_{Y^l|\mb{X}^l}$, usually presented as a pre-trained neural network, we evaluate $\mb{X}^u$ on $\widehat{\mathbb{P}}^l_{Y^l|\mb{X}^l}$ as $\widehat{\mb p}^l(\mb{X}^u) = \big(\widehat{\mathbb{P}}^l\big( Y^l=c | \mb{X}^l = \mb{X}^u \big) \big)_{c \in \mathcal{C}^u}$, then the empirical transfer leakage is computed as:
\begin{align}
	\label{eqn:emp_overall_leak}
	\widehat{\text{T-Leak}}( \mathbb{P}^u, \mathbb{P}^l ) & = \frac{2}{m(m-1)} \sum_{1\leq i< i' \leq m}  \widehat{\MMD}^2_{\mathcal{H}} \big( \widehat{\mb p}^l( \mathcal{U}_{Y_i^u} ),  \widehat{\mb p}^l( \mathcal{U}_{ Y^u_{i'} } ) \big) \nonumber \\
	& = \sum_{c, c' \in \mathcal{C}^u; c \neq c'} \frac{|\mathcal{U}_c| |\mathcal{U}_{c'}|}{m(m-1)} \widehat{\MMD}^2_{\mathcal{H}} \big( \widehat{\mb{p}}^l(\mathcal{U}_c), \widehat{\mb{p}}^l(\mathcal{U}_{c'}) \big),
\end{align}
where $\widehat{\mb p}^l( \mathcal{U}_c) = ( \widehat{\mb p}^l(\bm{X}^u), \mb{X}^u \in \mathcal{U}_c)$.

\subsection{Distinct difficulty benchmarks}
\label{sec:benchmark}
\begin{figure}[t]
\vspace{-0.0cm}
\centering
\includegraphics[width=0.8\linewidth]{figures/split.png}
\vspace{-0.15cm}
%\setlength{\tabcolsep}{2.8pt} % Default value: 6pt
\fontsize{9.1pt}{9.1pt}\selectfont
\caption{Illustration of how we construct different difficulty-level data settings.
Various colors symbolize various super classes.
Unlabeled classes are represented by a circle, while labeled classes are represented by a triangle.
We consider it as a simple case if both the labeled and unlabeled classes derive from the same super class. Conversely, it is the difficult case.}
\label{fig:splits}
\end{figure}
\begin{table}[]
    \centering
    % \fontsize{9.2pt}{9.2pt}\selectfont
    % \setlength{\tabcolsep}{6pt}
    \captionsetup{width=0.96\linewidth} 
    \caption{ 
    Detailed partition way of previous used benchmarks.
    }
\begin{tabular}{@{}lccll@{}}
\toprule
Dataset     & \# Known classes & \# Novel classes &  &  \\ \midrule
CIFAR100-20 & 80               & 20               &  &  \\
CIFAR100-50 & 50               & 50               &  &  \\
ImageNet    & 882              & 30               &  &  \\ \bottomrule
\end{tabular}
\label{tab:old benchmark}
\end{table}
The previous NCD benchmarks only focus on the number between labeled and unlabeled classes as the indicator of difficulty, as shown in Table~\ref{tab:old benchmark}.
% However, we also consider the  semantic similarity between labeled sets and unlabeled sets by leveraging the hierarchy of datasets.
However, as mention in \ref{lab:transfer leakage}, semantic similarity between labeled sets and unlabeled sets is the core to NCD's performance. 
Thus, we first verify it in CIFAR100~\cite{krizhevsky2009learning} and then conduct a three difficulty-level benchmark on ImageNet \cite{deng2009imagenet}. 

In CIFAR100~\cite{krizhevsky2009learning}, which consists of 20 superclasses, with 5 subclasses each, we first divide the data into two halves, each consisting of 10 superclasses. 
Then we divided subclasses into labeled and unlabeled classes for each superclass.
For example, in 1-4 split, one subclass is assigned as unlabeled while the other four are labeled classes.
Specifically, if both the labeled and unlabeled classes derive from the same superclass, we regard as easy case. Conversely, it is the difficult case, as shown in Figure \ref{fig:splits}.

Borrow the same idea from conducting different difficulty data settings on CIFAR100, we construct a new benchmark on ImageNet.
While this benchmark allows us to empirically prove our theory, it is based on a rather small dataset, and our approach of splitting the data into subsets essentially halves the amount of data the models are trained on. To also conduct our experiments in a more realistic setting, we propose a second benchmark based on the much larger ImageNet dataset \cite{deng2009imagenet}. While the ImageNet labels are based on the WordNet hierarchy \cite{miller1995wordnet}, this hierarchy is impractical as in \cite{santurkar2020breeds}. The reasons include the heavily imbalanced number of subclasses per superclass, the often very abstract nature of some superclasses, and the possibility of one subclasse having multiple superclasses. To address these issues, \cite{santurkar2020breeds} proposed an altered hierarchy as well as several ImageNet subsets based on it. One of them is the Entity30 benchmark, which consists of 240 ImageNet classes divided into 30 superclasses with 8 subclasses each. Based on Entity30, we split the data into three labeled and two unlabeled set similar to our first benchmark.


% \\
% hierarchy of dataset classes
% Thus, to systematically verify the impact the similarity between labeled sets and unlabeled sets has on NCD performance, we reclassify the labeled sets and unlabeled sets pair based on semantic similarity both CIFAR100 and ImageNet and propose a new benchmark on ImageNet.


% we propose two new benchmarks that contain different combinations of labeled sets and unlabeled sets of varying semantic similarity on both CIFAR100~\cite{krizhevsky2009learning} and ImageNet~\cite{deng2009imagenet}.

% Maybe we need a figure here to illustrate the dataset split?
% Numbers as words or numerals?

% \red{cifar100 is considered as verification, not benchmarks.}
% Our first benchmark in based on CIFAR100 \cite{krizhevsky2009learning}. To split the data into groups of similar classes, we leverage the hierarchy of the dataset, which consists of twenty superclasses, with five subclasses each. We first divide the data into two halves, each consisting of ten superclasses. Then, we split the subsets into a labeled and an unlabeled set, by assigning four subclasses of each superclass to the labeled set and the remaining class to the unlabeled set. In total, we now have two labeled subsets l1 and l2 and two unlabeled subsets u1 and u2, where l1 is closely related to u1 and l2 is closely related to u2. Additionally, we define a third labeled set l3, that contains half of the superclasses in l1 and half of the superclasses in l2. Under our assumptions it would be expected that combining u1 and l1 delivers better performance than the combining it with l2, with l3 somewhere in between. Thus, combining different splits of labeled and unlabeled classes allows us to investigate the impact semantic similarity has on \ac{ncd} performance.


\subsection{Experiments}
% \textbf{Datasets.} 
% \red{From UNO} \textbf{Datasets.} We first verify our assumptions on CIFAR100~\cite{krizhevsky2009learning} and then evaluate our method on both CIFAR100 and ImageNet~\cite{deng2009imagenet}. 
% We evaluate the performance of our method on
% three well-established NCD benchmarks following [8, 7],
% i.e., CIFAR10 [17], CIFAR100 [17] and ImageNet [5].
% Each dataset is divided into two subsets, the labeled set that
% contains labeled images belonging to a set of known classes,
% and an unlabeled set of novel classes for which we do not
% possess any supervision except for the number of classes.
% The details of the splits are shown in Tab. 1. Standard data
% splits used in the literature (1, 2 and 4 in Tab. 1) exhibit either (i) a small number of classes or (ii) a strong imbalance
% in the number of classes of the two subsets (the labeled set
% is much larger than the unlabeled set). However, these two
% assumptions do not hold in real-world scenarios, where the
% unlabeled data is far more abundant than its labeled counterpart. Hence, we introduce a new split that better approximates practical applications for NCD: CIFAR100-50. As
% shown in Tab. 1, CIFAR100-50 contains a large number of
% unlabeled classes (50), making the task more challenging.\\

% \textbf{Evaluation metrics.} \red{From RS, We adopt clustering accuracy (ACC) to evaluate the clustering performance
% of our approach. The ACC is defined as follow:}
% \begin{align*}
%     max {1}
% \end{align*}
% where yi and yi denote the ground-truth label and clustering assignment for each data point x
% u
% i ∈ Du
% respectively, and Sym(L) is the group permutations of L elements (this discounts the fact that the
% cluster indices may not be in the same order as the ground-truth labels). Permutations are optimized
% using the Hungarian algorithm (Kuhn, 1955).

\textbf{Experiment setup.}
We conduct four methods in our verified experiments, including K-means \cite{?}, DTC (The first formal NCD method), RS (typical method) and UNO (the-state-of-the-art) on ResNet18 \cite{?}.
\red{detail experiment settings.}


\textbf{Results.}
Table \ref{tab:old benchmark} shows the experiment results on CIFAR100, given an unlabeled set, 

For a fair comparison with existing methods, we use a ResNet18 [9] encoder for all datasets.  We pretrain our model for 200 epochs on
the labeled dataset and then train for 200 epochs in the discovery phase on both labeled and unlabeled datasets. For
both phases we use SGD with momentum as optimizer,
with linear warm-up and cosine annealing (lrbase = 0.1,
lrmin = 0.001), and weight decay 10−4
. The batch size
is always set to 512 for all experiments. Regarding the discovery phase, we use an overclustering factor m = 3 and
a n = 4 heads for both clustering and overclustering. The
temperature parameter τ is set to 0.1 for all softmax layers. For what concerns pseudo-labeling, we use the implementation of the Sinkhorn-Knopp algorithm [4] provided
by [2] and we inherit all the hyperparameters from [2], e.g.
n iter = 3 and  = 0.05.

\textbf{Results on CIFAR100} 

\textbf{Results on ImageNet}

\begin{table}[]
\centering
    % \fontsize{9.2pt}{9.2pt}\selectfont
    % \setlength{\tabcolsep}{6pt}
    % \captionsetup{width=0.96\linewidth} 
    \caption{ 
    Comparison among different correlation between unlabeled sets and labeled sets on CIFAR100. 
    U1 and U2 denote different unlabeled sets.
    Similarly, L1 and L2 represent different labeled sets.
    (U1, L1) are belong to the same super class while (U2, L2) share the other same super class.
    Thus, 1, L1) and (U2, L2) are close semantically, but (U1, L2) and (U2, L1) are far apart semantically.
    As for the same unlabeled set, close semantic pair have a higher performance than the far one.
    % More experiments results are in supplementary.
    }
    
\begin{tabular}{@{}lcccc@{}}
\toprule
\multirow{2}{*}{} & \multicolumn{2}{c}{U1} & \multicolumn{2}{c}{U2} \\ \cmidrule(l){2-3}   \cmidrule(l){4-5} 
                     & Close (U1,L1)     & Far (U1,L2)     & Far (U2,L1)     & Close (U2,L2)    \\ 
%   {T-leakage}      & ? & ? & ? & ? \\                         
                         \midrule
   K-means                  & 63.42             & 51.16           & 52.24           & 72.78             \\
DTC                      & 74.76             & 57.16           & 62.24           & 80.38             \\
RS                       & 76.72             & 75.68           & 75.12           & 82.28             \\
UNO                      & 87.54             & 85.36           & 85.66           & 91.22             \\ 
        \vspace{-0.25cm}
		&\\
		\hline
		\vspace{-0.25cm}
		&\\
T-leakage & 42.12 & 26.58 & 28.14 & 50.63 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[]
\centering
    % \fontsize{9.2pt}{9.2pt}\selectfont
    % \setlength{\tabcolsep}{6pt}
    % \captionsetup{width=0.96\linewidth} 
    \caption{ 
    Comparison among different correlation between unlabeled sets and labeled sets on our benchmark.
    }
\begin{tabular}{@{}lcccccc@{}}
\toprule
\multirow{2}{*}{Methods} & \multicolumn{3}{c}{Unlabeled set 1}           & \multicolumn{3}{c}{Unlabeled set 2}            \\ \cmidrule(l){2-4} \cmidrule(l){5-7} 
                         & close (u1,l1) & middle(u1, l3) & far (u1,l2)  & far (u2,l1)  & middle(u2, l3) & strong (u2,l2) \\ \midrule
K-means                  & 60.98 ± 0.95  & 55.56 ± 1.06   & 44.00 ± 0.97 & 39.12 ± 0.61 & 45.73 ± 0.55   & 55.11 ± 1.59   \\
DTC                      & 43.31 ± 2.58  & 35.60 ± 2.95   & 32.22 ± 1.90 & 21.29 ± 2.73 & 15.28 ± 3.44   & 28.97 ± 1.84   \\
RS                       & ?             & \textbf{?}     & \textbf{?}   & \textbf{?}   & \textbf{?}     & ?              \\
UNO                      & 83.89 ± 1.24  & 80.95 ± 1.23   & 77.19 ± 1.81 & 77.45 ± 1.55 & 82.02 ± 3.69   & 88.35 ± 2.57  
\\ \bottomrule
\end{tabular}
\label{tab:new_benchmark}
\end{table}



% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \begin{table}[]
% \centering
% \begin{tabular}{@{}ccccccc@{}}
% \toprule
% \multirow{2}{*}{Methods}                       & \multicolumn{3}{c}{(L1,U1) Strong correlation}   & \multicolumn{3}{c}{(L2,U1) Weak correlation}     \\ \cmidrule(l){2-4} \cmidrule(l){5-7} 
%                                               & ACC            & NMI            & ARI            & ACC            & NMI            & ARI            \\ \cmidrule(r){1-1}
% K-means                                        & \textbf{63.42} & \textbf{57.08} & \textbf{46.65} & 51.16          & 36.88          & 26.83          \\
% PCA+K-means                                    & \textbf{67.86} & \textbf{55.98} & \textbf{47.68} & 48.8           & 34.46          & 25.98          \\
% DTC                                            & \textbf{74.76} & \textbf{67.35} & \textbf{60.47} & 57.16          & 47.02          & 36.51          \\ 
% RS                                             & \textbf{76.72} & \textbf{72.18} & \textbf{66.2}  & 75.68          & 71.44          & 57.29          \\
% UNO                                            & \textbf{87.54} & \textbf{80.78} & \textbf{77.8}  & 85.36          & 79.54          & 76.37          \\ \midrule
% \multirow{2}{*}{Methods}  & \multicolumn{3}{c}{(L1,U2) Weak correlation}    & \multicolumn{3}{c}{(L2,U2) Strong correlation}  
%     \\ \cmidrule(l){2-4} \cmidrule(l){5-7} 
%                                               & ACC            & NMI            & ARI            & ACC            & NMI            & ARI            \\ 
%                                               \cmidrule(r){1-1}
% K-means                                        & 52.24          & 40.08          & 30.08          & \textbf{72.78} & \textbf{58.98} & \textbf{52.07} \\
% PCA+K-means                                    & 50.92          & 38.4           & 29.05          & \textbf{70.82} & \textbf{57.85} & \textbf{49.94} \\
% DTC                                            & 62.24          & 51.72          & 44.61          & \textbf{80.38} & \textbf{70.04} & \textbf{65.66} \\
% RS                                             & 75.12          & 65.34          & 56.98          & \textbf{82.28} & \textbf{73.47} & \textbf{63.9}  \\
% UNO                                            & 85.66          & 74.44          & 72.47          & \textbf{91.22} & \textbf{81.35} & \textbf{81.79} \\ \bottomrule
% \end{tabular}
% \end{table}

% \begin{table}[]
% 	\caption{
% 	    Results on CIFAR100's U1 unlabeled set. All methods are use ResNet18 as pre trained model.
% 	    Model\_L1 and Model\_L2 are first trained in L1 labeled set and L2 labeled set, respectively.
	    
% 	}
% 	%\vspace{-0.10cm}
% 	\centering
% 	%\fontsize{9.5pt}{9.5pt}\selectfont
% 	%\setlength{\tabcolsep}{16.5pt} % Default value: 6pt
% \begin{tabular}{@{}lcccccc@{}}
% \toprule
% \multirow{2}{*}{Methods}        & \multicolumn{3}{c}{Model\_L1(ACC: 77.80)}                           & \multicolumn{3}{c}{Model\_L2(76.05)}                               \\ 	\cmidrule(lr){2-4}
% 		\cmidrule(lr){5-7}
%                                 & acc                  & nmi                  & ari                  & acc                  & nmi                  & ari                  \\ \cmidrule(r){1-1}
% \multicolumn{1}{l}{K-means}     & \textbf{63.42}       & \textbf{57.08}       & \textbf{46.65}       & 51.16                & 36.88                & 26.83                \\
% \multicolumn{1}{l}{K-means+PCA} & \textbf{67.86}       & \textbf{55.98}       & \textbf{47.68}       & 48.80                 & 34.46                & 25.98                \\
% \multicolumn{1}{l}{DTC}         & \textbf{74.76}       & \textbf{67.35}       & \textbf{60.47}       & 57.16                & 47.02                & 36.51                \\

%  \bottomrule
% \end{tabular}
% \end{table}

% \begin{table}[]
% 	\caption{
% 	    Results on CIFAR100's U2 unlabeled set. All methods are use ResNet18 as pre trained model.
% 	    Model\_L1 and Model\_L2 are first trained in L1 labeled set and L2 labeled set, respectively.
	    
% 	}
% 	%\vspace{-0.10cm}
% 	\centering
% 	%\fontsize{9.5pt}{9.5pt}\selectfont
% 	%\setlength{\tabcolsep}{16.5pt} % Default value: 6pt
% \begin{tabular}{@{}ccccccc@{}}
% \toprule
% \multirow{2}{*}{Methods}        & \multicolumn{3}{c}{Model\_L1(ACC: 77.8)}                           & \multicolumn{3}{c}{Model\_L2(76.05)}                               \\ \cmidrule(l){2-7} 
%                                 & acc                  & nmi                  & ari                  & acc                  & nmi                  & ari                  \\ \cmidrule(r){1-1}
% \multicolumn{1}{l}{K-means}     & \textbf{52.24}       & \textbf{40.08}       & \textbf{30.08}       & \textbf{72.78}       & 58.98                & 52.07                \\
% \multicolumn{1}{l}{K-means+\textmin{PCA}} & \textbf{50.92}       & \textbf{38.40}        & \textbf{29.05}       & \textbf{70.82}       & 57.85                & 49.94                \\
% \multicolumn{1}{l}{DTC}         & \textbf{62.24}       & \textbf{51.72}       & \textbf{44.61}       & \textbf{80.38}       & 70.04                & 65.66                \\
% \bottomrule
% \end{tabular}
% \end{table}




==> sections/04_second.tex <==
\section{How each element of the labeled set impact the unlabeled set's performance?}

\subsection{The impact from supervised pre-trained model}

\subsection{The impact from images without labels}

\subsection{Our Proposed method}

\begin{table}[t!]
\centering
    \fontsize{9.2pt}{9.2pt}\selectfont
    % \setlength{\tabcolsep}{6pt}
    % \captionsetup{width=0.96\linewidth} 
    \caption{ 
    Comparison among only use unlabeled set (\mathrm{$X_u$}), unlabeled set and labeled data without labeles ($X_u + X_l$), and unlabeled set and labeled data with labeles($X_u + (X_l, Y_l)$).
    We conduct experiments on CIFAR100, 50-50 spilit as \cite{fini2021unified} and ImageNet three difficulty-level benchmarks \ref{sec:benchmark}, easy (L1-U1), middle (L3-U1) and hard (L2-U1).
    \red{conclusion}
    }
\begin{tabular}{llcccc}
\toprule
\multicolumn{1}{l}{Methods}                     &
\multicolumn{1}{l}{ } &
\multicolumn{1}{c}{CIFAR100} & \multicolumn{1}{c}{ImageNet(easy)} & \multicolumn{1}{c}{ImageNet(middle)} & \multicolumn{1}{c}{ImageNet(hard)} \\
\hline
\multirow{3}{*}{UNO(avg)}  & $X_u$               &                                      &                                          &                                          &                                          \\
                          & $X_u+X_l$        &                                      &                                          &                                          &                                          \\
                          & $X_u + (X_l,Y_l)$ &                                      &                                          &                                          &                                          \\
\hline
\multirow{3}{*}{UNO(Best)} & $X_u$               &                                      &                                          &                                          &                                          \\
                          & $X_u+X_l$       &                                      &                                          &                                          &                                          \\
                          & $X_u + (X_l,Y_l)$ &                                      &                                          &                                          &                                          \\
\hline
\multirow{3}{*}{RS}        & $X_u$               &                                      &                                          &                                          &                                          \\
                          & $X_u+X_l$       &                                      &                                          &                                          &                                          \\
                          & $X_u + (X_l,Y_l)$ &                                      &                                          &                                          &                                          \\
\hline
\multirow{3}{*}{RS+}       & $X_u$               &                                      &                                          &                                          &                                          \\
                          & $X_u+X_l$       &                                      &                                          &                                          &                                          \\
                          & $X_u + (X_l,Y_l)$ &                                      &                                          &                                          &                                          \\
\hline
\multirow{3}{*}{Ours}      & $X_u$               &                                      &                                          &                                          &                                          \\
                          & $X_u+X_l$       &                                      &                                          &                                          &                                          \\
                          & $X_u + (X_l,Y_l)$ &                                      &                                          &                                          &                                          \\
\hline
\multirow{3}{*}{K-means}   & $X_u$               &                                      &                                          &                                          &                                          \\
                          & $X_u+X_l$       &                                      &                                          &                                          &                                          \\
                          & $X_u + (X_l,Y_l)$ &                                      &                                          &                                          & 
                          \\
\bottomrule
\end{tabular}
\label{tab:x+y}
\end{table}

==> sections/05_experiments.tex <==
\section{Experiments}



\subsection{Experiment Setup}
\red{From UNO} \textbf{Datasets.} We first verify our assumptions on CIFAR100~\cite{krizhevsky2009learning} and then evaluate our method on both CIFAR100 and ImageNet~\cite{deng2009imagenet}. 
We evaluate the performance of our method on
three well-established NCD benchmarks following [8, 7],
i.e., CIFAR10 [17], CIFAR100 [17] and ImageNet [5].
Each dataset is divided into two subsets, the labeled set that
contains labeled images belonging to a set of known classes,
and an unlabeled set of novel classes for which we do not
possess any supervision except for the number of classes.
The details of the splits are shown in Tab. 1. Standard data
splits used in the literature (1, 2 and 4 in Tab. 1) exhibit either (i) a small number of classes or (ii) a strong imbalance
in the number of classes of the two subsets (the labeled set
is much larger than the unlabeled set). However, these two
assumptions do not hold in real-world scenarios, where the
unlabeled data is far more abundant than its labeled counterpart. Hence, we introduce a new split that better approximates practical applications for NCD: CIFAR100-50. As
shown in Tab. 1, CIFAR100-50 contains a large number of
unlabeled classes (50), making the task more challenging.\\

\textbf{Evaluation metrics.} \red{From RS, We adopt clustering accuracy (ACC) to evaluate the clustering performance
of our approach. The ACC is defined as follow:}
\begin{align*}
    max {1}
\end{align*}
where yi and yi denote the ground-truth label and clustering assignment for each data point x
u
i ∈ Du
respectively, and Sym(L) is the group permutations of L elements (this discounts the fact that the
cluster indices may not be in the same order as the ground-truth labels). Permutations are optimized
using the Hungarian algorithm (Kuhn, 1955).\\

\textbf{Implementation details.} \red{from uno} For a fair comparison with existing methods, we use a ResNet18 [9] encoder for all datasets.  We pretrain our model for 200 epochs on
the labeled dataset and then train for 200 epochs in the discovery phase on both labeled and unlabeled datasets. For
both phases we use SGD with momentum as optimizer,
with linear warm-up and cosine annealing (lrbase = 0.1,
lrmin = 0.001), and weight decay 10−4
. The batch size
is always set to 512 for all experiments. Regarding the discovery phase, we use an overclustering factor m = 3 and
a n = 4 heads for both clustering and overclustering. The
temperature parameter τ is set to 0.1 for all softmax layers. For what concerns pseudo-labeling, we use the implementation of the Sinkhorn-Knopp algorithm [4] provided
by [2] and we inherit all the hyperparameters from [2], e.g.
n iter = 3 and  = 0.05.

\subsection{Assumptions Verification}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[]
\centering
\begin{tabular}{@{}ccccccc@{}}
\toprule
\multirow{2}{*}{Methods}                       & \multicolumn{3}{c}{(L1,U1) Strong correlation}   & \multicolumn{3}{c}{(L2,U1) Weak correlation}     \\ \cmidrule(l){2-4} \cmidrule(l){5-7} 
                                               & ACC            & NMI            & ARI            & ACC            & NMI            & ARI            \\ \cmidrule(r){1-1}
K-means                                        & \textbf{63.42} & \textbf{57.08} & \textbf{46.65} & 51.16          & 36.88          & 26.83          \\
PCA+K-means                                    & \textbf{67.86} & \textbf{55.98} & \textbf{47.68} & 48.8           & 34.46          & 25.98          \\
DTC                                            & \textbf{74.76} & \textbf{67.35} & \textbf{60.47} & 57.16          & 47.02          & 36.51          \\ 
RS                                             & \textbf{76.72} & \textbf{72.18} & \textbf{66.2}  & 75.68          & 71.44          & 57.29          \\
UNO                                            & \textbf{87.54} & \textbf{80.78} & \textbf{77.8}  & 85.36          & 79.54          & 76.37          \\ \midrule
\multirow{2}{*}{Methods}  & \multicolumn{3}{c}{(L1,U2) Weak correlation}    & \multicolumn{3}{c}{(L2,U2) Strong correlation}  
    \\ \cmidrule(l){2-4} \cmidrule(l){5-7} 
                                               & ACC            & NMI            & ARI            & ACC            & NMI            & ARI            \\ 
                                               \cmidrule(r){1-1}
K-means                                        & 52.24          & 40.08          & 30.08          & \textbf{72.78} & \textbf{58.98} & \textbf{52.07} \\
PCA+K-means                                    & 50.92          & 38.4           & 29.05          & \textbf{70.82} & \textbf{57.85} & \textbf{49.94} \\
DTC                                            & 62.24          & 51.72          & 44.61          & \textbf{80.38} & \textbf{70.04} & \textbf{65.66} \\
RS                                             & 75.12          & 65.34          & 56.98          & \textbf{82.28} & \textbf{73.47} & \textbf{63.9}  \\
UNO                                            & 85.66          & 74.44          & 72.47          & \textbf{91.22} & \textbf{81.35} & \textbf{81.79} \\ \bottomrule
\end{tabular}
\end{table}

% \begin{table}[]
% 	\caption{
% 	    Results on CIFAR100's U1 unlabeled set. All methods are use ResNet18 as pre trained model.
% 	    Model\_L1 and Model\_L2 are first trained in L1 labeled set and L2 labeled set, respectively.
	    
% 	}
% 	%\vspace{-0.10cm}
% 	\centering
% 	%\fontsize{9.5pt}{9.5pt}\selectfont
% 	%\setlength{\tabcolsep}{16.5pt} % Default value: 6pt
% \begin{tabular}{@{}lcccccc@{}}
% \toprule
% \multirow{2}{*}{Methods}        & \multicolumn{3}{c}{Model\_L1(ACC: 77.80)}                           & \multicolumn{3}{c}{Model\_L2(76.05)}                               \\ 	\cmidrule(lr){2-4}
% 		\cmidrule(lr){5-7}
%                                 & acc                  & nmi                  & ari                  & acc                  & nmi                  & ari                  \\ \cmidrule(r){1-1}
% \multicolumn{1}{l}{K-means}     & \textbf{63.42}       & \textbf{57.08}       & \textbf{46.65}       & 51.16                & 36.88                & 26.83                \\
% \multicolumn{1}{l}{K-means+PCA} & \textbf{67.86}       & \textbf{55.98}       & \textbf{47.68}       & 48.80                 & 34.46                & 25.98                \\
% \multicolumn{1}{l}{DTC}         & \textbf{74.76}       & \textbf{67.35}       & \textbf{60.47}       & 57.16                & 47.02                & 36.51                \\

%  \bottomrule
% \end{tabular}
% \end{table}

% \begin{table}[]
% 	\caption{
% 	    Results on CIFAR100's U2 unlabeled set. All methods are use ResNet18 as pre trained model.
% 	    Model\_L1 and Model\_L2 are first trained in L1 labeled set and L2 labeled set, respectively.
	    
% 	}
% 	%\vspace{-0.10cm}
% 	\centering
% 	%\fontsize{9.5pt}{9.5pt}\selectfont
% 	%\setlength{\tabcolsep}{16.5pt} % Default value: 6pt
% \begin{tabular}{@{}ccccccc@{}}
% \toprule
% \multirow{2}{*}{Methods}        & \multicolumn{3}{c}{Model\_L1(ACC: 77.8)}                           & \multicolumn{3}{c}{Model\_L2(76.05)}                               \\ \cmidrule(l){2-7} 
%                                 & acc                  & nmi                  & ari                  & acc                  & nmi                  & ari                  \\ \cmidrule(r){1-1}
% \multicolumn{1}{l}{K-means}     & \textbf{52.24}       & \textbf{40.08}       & \textbf{30.08}       & \textbf{72.78}       & 58.98                & 52.07                \\
% \multicolumn{1}{l}{K-means+\textmin{PCA}} & \textbf{50.92}       & \textbf{38.40}        & \textbf{29.05}       & \textbf{70.82}       & 57.85                & 49.94                \\
% \multicolumn{1}{l}{DTC}         & \textbf{62.24}       & \textbf{51.72}       & \textbf{44.61}       & \textbf{80.38}       & 70.04                & 65.66                \\
% \bottomrule
% \end{tabular}
% \end{table}

\subsection{Ablation Study}

\subsection{Comparison with the state-of-the-art}

\subsection{Qualitative Results}

% \subsection{Benchmarks}


==> sections/06_discussion.tex <==
\section{Discussion}


==> sections/07_checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section [].}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}{}
  \item Did you describe the limitations of your work?
    \answerYes{}{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{We think there are no negative societal impacts of our work, that need considering.}{}{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{See Section 4.3}{}{}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{See Appendix}{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{See experiment settings and appendix.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See experiment setttins}{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{See Tables and experiment settings}{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Section 3.3}{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}{}
  \item Did you mention the license of the assets?
    \answerYes{}{}{}{}{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}{}{}{}{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}{}{}{}{}{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}{}
\end{enumerate}


\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> sections/Information_leakage.tex <==
\section{Information leakage in NCD}
In this section, we introduce a formal framework of the novel class discovery (NCD). To proceed, let $(\mb{X}^l, Y^l)$ and $(\mb{X}^u, Y^u)$ be random samples under the \emph{labeled/unlabeled probability measures} $\mathbb{P}^l$ and $\mathbb{P}^u$, respectively.
Here $\mb{X}^l \in \mathcal{X}^l \subset \mathbb{R}^d$ and $\mb{X}^u \in \mathcal{X}^u \subset \mathbb{R}^d$ are the labeled/unlabeled feature vectors. $Y^l \in \mathcal{C}^l$ and $Y^u \in \mathcal{C}^u$ are the labels of labeled/unlabeled data, where $\mathcal{C}^l / \mathcal{C}^u$ is the label set under the labeled probability measure $\mathbb{P}^l / \mathbb{P}^u$.
There are labeled dataset $\mathcal{L}_n = (\mb{X}_i^{l}, Y_i^{l})_{i=1, \cdots, n}$ independently drawn from the labeled probability measure $\mathbb{P}^{l}$, and unlabeled dataset $ \mathcal{U}_m = (\mb{X}_i^{u})_{i=1, \cdot, m}$ independently drawn from the unlabeled probability measure $\mathbb{P}_{\mb{X}}^u$. Our primary goal is to make prediction to $Y^u_i$ under the probability measure $\mathbb{P}^{u}$ given $\mb{X}_i^{u}$. We now give a general definition of NCD.

\begin{definition}[Novel class discovery]
	Given a labeled probability measure $\mathbb{P}^l$ on $\mathcal{X}^l \times \mathcal{C}^l$, an unlabeled probability measure $\mathbb{P}^u$ on $\mathcal{X}^u \times \mathcal{C}^u$, and a labeled dataset $\mathcal{L}_n$ and an unlabeled dataset $\mathcal{U}_m$, novel class discovery aims to predict the labels of the unlabeled dataset based on $\mathcal{L}_n$ and $\mathcal{U}_m$, where $\mathcal{C}^u \neq \mathcal{C}^l$.
\end{definition}

In general, NCD is a subgroup of transfer learning, with both domains and tasks are different. Yet, it has own distinct characteristics in the existence of new classes on the unlabeled dataset. In Figure \red{add figure}, we summarize the relationship/difference among three major learning paradigms (with both labeled and unlabeled datasets): NCD, semi-supervised learning and transductive transfer learning.

% Then, the training samples $\mathcal{D}_\old = (\mb{X}_{\old,i}, Y_{\old,i})^{n_\old}_{i=1}$ are independent and identically drawn from the old probability measure $\mathbb{P}_\old$ on $(\mb{X}_l, Y_l)$. Note that $\mathcal{C}^{(l)}$ may not be fully observed by $\mathcal{D}_\old$, thus we denote $\mathcal{C}^{\text{sub}}_{\old} = \text{set}\{ (Y_i)_{i=1}^n \}$ to clarify. 
% For the new distribution, we observe $n_\new$ independent and identically distributed unlabeled data $( \mb{X}_{\new, l})_{l=1}^m$. The new class with respect to the training sample $\mathcal{D}_\old$ is defined as $\mathcal{C}^u / \mathcal{C}^{\text{sub}}_{\old}$.
\red{add more about the marginal information, and $\mathbb{P}_{Y|\mb{X}}$ only.}

Note that it is critical to measure the similarity between $\mathbb{P}^l$ and $\mathbb{P}^u$. As indicated in Figure \red{???}, NCD degenerates to the classical SSL when $\mathbb{P}^l = \mathbb{P}^u$, or the transductive transfer learning if $\mathbb{P}_{Y|\mb{X}}^l = \mathbb{P}_{Y|\mb{X}}^u$. Moreover, in practice, there are many pairs of labeled and unlabeled dataset to choose from. For example, fixing the unlabeled dataset as CIFAR-100, we can use CIFAR-10, CIFAR-50 or Image-NET as the labeled dataset. Certainly, different pairs of labeled/unlabeled datasets yield various predictive performance. This leads to the following questions: 
\begin{itemize}
	\item How can we tell the overall \textit{difficulty} of NCD under $\mathbb{P}^u$ based on unlabeled dataset $\mathcal{U}_m$?
	\item How much does the labeled dataset $\mathcal{L}_n$ under $\mathbb{P}^l$ can help to predict the label under $\mathbb{P}^u$?
\end{itemize}
 To address the questions, we propose the concept of \textit{leakage} to measure the difficulty of NCD. Specifically, the first question concerns the overall difficulty of NCD under an unsupervised manner, which predicts labels solely based on marginal information of $\mb{X}^{u}$, is highly related to the discriminative information leaked in the marginal distribution, namely \textit{overall leakage}. For the second question, we introduce \textit{transfer leakage} to quantify the discriminative information in $\mathbb{P}^u$ leaked in $\mathbb{P}^l$, that is, how much information we can leverage from the labeled dataset to help improve the performance of the unlabeled dataset.

It is worth to point out that investigation of the questions not only can help us to construct benchmark dataset for fair numerical comparison of existing methods (see Section \red{???}), but also inspire our proposed method yielding state-of-the-art performance in NCD (see Section \red{???}).

\subsection{Overall leakage}
\red{Change to IPM to make it more general.}
To quantify the \emph{overall leakage} under the probability measure $\mathbb{P}^u$, we turn to measure the discrepancy of $\mb{X}^{u}$ given different labels $Y^u = c; (c \in \mathcal{C}^{u})$. For instance, given two labels $c, c' \in \mathcal{C}^u$, if there exists a transformation $h(\cdot)$ such that the distributions of $h(\mb{X}^u) | Y^u = c$ and $h(\mb{X}^u) | Y^u = c'$ are easily separable (or distance is large), then it is potential feasible to discriminate $c$ and $c'$ under an unsupervised manner. To this end, we introduce Maximum Mean Discrepancy (MMD; \citep{gretton2012kernel}) or Wasserstein-1 distance (\cite{pmlr-v70-arjovsky17a}) to quality the discrepancy of two distributions:
\begin{align}
	\label{def:mmd}
	\MMD_\mathcal{H} \big( \mathbb{P}^u_{\mb{X}^u | Y^u=c'}, \mathbb{P}^u_{\mb{X}^u | Y^u = c} \big) := \sup_{h \in \mathcal{H}} \Big( \mathbb{E}\big( h( \mb{X}^u) \mid Y^u = c \big) - \mathbb{E}\big( h( \mb{X}^u) \mid Y^u = c'\big) \Big)
\end{align}
where $\mathcal{H}$ is a class of functions $h: \mathcal{X}^u \to \mathbb{R}$, which is usually specified as the unit ball in a reproducing kernel Hilbert Space (RKHS), or a deep neural network as in W-GAN \citep{pmlr-v70-arjovsky17a}.
From \eqref{def:mmd}, when $\MMD$ is large, it provides a relatively large possibility to find a good transformation on $\mb{X}^u$ discriminating labels in an unsupervised manner. 

% \noindent \textbf{Remark.} In \eqref{def:mmd}, we use a generative model $\mathbb{Q}_{\mb{X}^u | Y^u=c}$ to quantify the overall leakage, one may suggest using a discriminative model $\mathbb{Q}( Y^u = c| \mb{X}^u ); (c \in \mathcal{C}^u)$ to quality the leakage of the prediction under $\mathbb{Q}$. It is sensible in supervised learning, when $(\mb{X}^u, Y^u)$ is observed in training set. In our case, our goal to measure the leakage based on an unsupervised manner, where the discrepancy of $\mathbb{Q}_{\mb{X}^u | Y^u=c}$ is more reasonable.

For multi-class discrepancy, we mimic the one-vs-rest nature by taking the minimum discrepancy over all rest classes, which takes the discrepancy to the closest class. Taken together, the overall leakage is defined as follows.
\begin{definition}[Overall leakage]
	\label{def:O-leak}
	The overall \textit{leakage} of NCD prediction on $\mathbb{P}^u$ is defined as 
	\begin{equation}
	\text{O-Leak}( \mathbb{P}^u ) = \mathbb{E} \Big( \MMD^2 \big( \mathbb{P}^u_{\mb{X}^u | Y^u }, \mathbb{P}^u_{\widetilde{\mb{X}}^u | \widetilde{Y}^u } \big) \Big),
	\end{equation}
	where $(\mb{X}^u, Y^u), (\widetilde{\mb{X}}^u, \widetilde{Y}^u) \sim \mathbb{P}^u$ are independent copies under $\mathbb{P}^u$, and the expectation is taken with respect to $Y^u$ and $\widetilde{Y}^u$. 
\end{definition}

\begin{lemma}
	\label{lemma:ol-zero}
	$\text{O-Leak}( \mathbb{P}^u ) = 0$ if and only if $Y^u$ is independent with $\mb{X}^u$, that is, for any $c \in \mathcal{C}^u$:
	$$
	\mathbb{P}^u( Y^u = c \mid \mb{X}^u ) = \mathbb{P}^u(Y^u = c).
	$$
\end{lemma}
Lemma \ref{lemma:ol-zero} indicates that if there is no overall leakage on $\mb{X}^u$ when predicting $Y^u$, then the best way to predict $Y^u$ given $\mb{X}^u$ is majority voting on $Y^u$. In practice, NCD dataset are often pre-balanced, that is, $\mathbb{P}^u(Y^u = c) = 1/|\mathcal{C}^u|$ for all $c \in \mathcal{C}^u$. 
% Then, \eqref{eqn:ol_gen_model} can be replaced as $\mathbb{P}^u(Y^u=c|\mb{X}^u) = \mathbb{P}(Y^u = c' | \mb{X}^u)$, and the best prediction is random guess. 
Therefore, the proposed overall leakage is a reasonable criterion to measure the predictive information leakage on $\mb{X}^u$, and the overall difficulty of NCD.


Suppose the labels $(Y^u_i)_{i=1, \cdot, m}$ for the unlabeled dataset are observed, denote $\mathcal{U}_c = \{ \mb{X}^u_i \in \mathcal{U}_m: Y_i^u = c\}$ as the sub-sample set under label $c$, the \textit{overall leakage} is empirically evaluated as 
\begin{align}
	\label{eqn:emp_overall_leak}
	\widehat{\text{O-Leak}}( \mathbb{P}^u ) & = \frac{2}{m(m-1)} \sum_{1 \leq i < i' \leq m} \widehat{\MMD}^2_{\mathcal{H}} \big( \mathcal{U}_{Y_i^u}, \mathcal{U}_{Y^u_{i'}} \big) = \sum_{c, c' \in \mathcal{C}^u; c \neq c'} \frac{|\mathcal{U}_c||\mathcal{U}_{c'}|}{m(m-1)} \widehat{\MMD}^2_{\mathcal{H}} \big( \mathcal{U}_c, \mathcal{U}_{c'} \big),
\end{align}
where $\widehat{\MMD}_{\mathcal{H}}$ is an empirical evaluation of MMD based on $\mathcal{H}$. For example, 
letting $\mathcal{H} = \mathcal{H}_K$ as a RKHS, we have
\begin{align}
	\label{eqn:emp_mmd}
	\widehat{\MMD}^2_{\mathcal{H}} ( \mathcal{U}_{c}, \mathcal{U}_{c'}) & = \frac{1}{|\mathcal{U}_{c}| \big( |\mathcal{U}_{c}| - 1 \big)} \sum_{ \mb{X}, \mb{X}' \in \mathcal{U}_{c}; \mb{X} \neq \mb{X}'} k( \mb{X}, \mb{X}' ) + \frac{1}{|\mathcal{U}_{c'}| \big( |\mathcal{U}_{c'}| - 1 \big)} \sum_{ \mb{X}, \mb{X}' \in \mathcal{U}_{c'}; \mb{X} \neq \mb{X}'} k( \mb{X}, \mb{X}' ) \nonumber \\ 
	& \quad - \frac{1}{|\mathcal{U}_{c}| |\mathcal{U}_{c'}| } \sum_{ \mb{X} \in \mathcal{U}_{c} } \sum_{ \mb{X}' \in \mathcal{U}_{c'}} k( \mb{X}, \mb{X}'),
\end{align}
where $k(\cdot, \cdot)$ is a reproducing kernel, such as Gaussian kernel. Note that a large $\widehat{\text{O-Leak}}_m(\mathbb{P}^u )$ implies that there is clear discrepancy on $\mb{X}^u$ among different classes, which indicates potential capability of unsupervised learning with $\mb{X}^u$ predicting its label. In practice, $\mb{X}^u$ is usually replaced by a latent feature from representation learning.

\subsection{Transfer leakage}
For unsupervised learning, it is usually quite difficult to learn such as good transformation solely based on $\mb{X}^u$. Instead, NCD takes account of the conditional probability $\mathbb{P}^l_{Y | \mb{X} }$ (usually presented by a pre-trained neural network) from a labeled dataset to help construct a transformation. Thus, we consider \emph{transfer leakage} of $\mathbb{P}^l$ on $\mathbb{P}^u$.

The main idea is to quantify the discrepancy of $\mathbb{P}^l_{Y|\mb{X}}$ on $\mb{X}^u$ under the new measure $\mathbb{P}^u$. Then, \emph{transfer leakage} can be defined as follows.

\begin{definition}[Transfer leakage]
	\label{def:T-leak}
	The transfer leakage of NCD prediction under $\mathbb{P}^u$ based on the labeled conditional probability $\mathbb{P}^l_{Y^l|\mb{X}^l}$ is 
	\begin{equation}
	\text{T-Leak}( \mathbb{P}^u, \mathbb{P}^l ) = \mathbb{E} \Big( \MMD^2 \big( \mathbb{P}^u_{ \mb{p}^l(\mb{X}) | Y }, \mathbb{P}^u_{\mb{p}^l(\mb{X}') \mid Y'} \big) \Big),
	\end{equation}
	where $(\mb{X}, Y), (\mb{X}', Y') \sim \mathbb{P}^u$ are independent copies, the expectation is taken with respect to $Y$ and $Y'$ under $\mathbb{P}^u$, and $\mb{p}^l(\mb{X}^u)$ is the conditional probability under $\mathbb{P}^l_{Y|\mb{X}}$ on an unlabeled instance $\mb{X}^u$, which is defined as
	$$
	\mb{p}^l(\mb{x}) = \big(\mathbb{P}^l\big( Y^l=c \mid \mb{X}^l = \mb{x} \big) \big)_{c \in \mathcal{C}^l}.
	$$
\end{definition}
With the similar manner in Definition \ref{def:O-leak}, the definition of transfer leakage is to measure the discrepancy of $\mb{p}(\mb{X}^u)$ under different new classes of $\mathbb{P}^u$, which indicates the  informative leakage of $\mathbb{P}^u$ on $\mathbb{P}^l$, and potential capability of transferring information from $\mathbb{P}^l$ to $\mathbb{P}^u$.

\begin{lemma}
	\label{lemma:tl-zero}
	$\text{T-Leak}( \mathbb{P}^u, \mathbb{P}^l ) = 0$ if and only if $Y^u$ is independent with $\mb{p}^l(\mb{X}^u)$, that is, for any $c \in \mathcal{C}^u$:
	\begin{equation}
		\label{eqn:tl-indep}
		\mathbb{P}^u\big( Y^u = c \mid \mb{p}^l(\mb{X}^u) \big) = \mathbb{P}^u(Y^u = c).
	\end{equation}
	Moreover, if $ \mathbb{P}^u = \mathbb{P}^l$, then \eqref{eqn:tl-indep} can be replaced as:
	$$
	\mathbb{P}^l\big( Y^l = c \mid \mb{X}^l \big) = \mathbb{P}^l(Y^l = c).
	$$
\end{lemma}

Given an estimated conditional probability $\widehat{\mathbb{P}}^l_{Y^l|\mb{X}^l}$, usually presented as a pre-trained neural network, we evaluate $\mb{X}^u$ on $\widehat{\mathbb{P}}^l_{Y^l|\mb{X}^l}$ as $\widehat{\mb p}^l(\mb{X}^u) = \big(\widehat{\mathbb{P}}^l\big( Y^l=c | \mb{X}^l = \mb{X}^u \big) \big)_{c \in \mathcal{C}^u}$, then the empirical transfer leakage is computed as
\begin{align}
	\label{eqn:emp_overall_leak}
	\widehat{\text{T-Leak}}( \mathbb{P}^u, \mathbb{P}^l ) & = \frac{2}{m(m-1)} \sum_{1\leq i< i' \leq m}  \widehat{\MMD}^2_{\mathcal{H}} \big( \widehat{\mb p}^l( \mathcal{U}_{Y_i^u} ),  \widehat{\mb p}^l( \mathcal{U}_{ Y^u_{i'} } ) \big) \nonumber \\
	& = \sum_{c, c' \in \mathcal{C}^u; c \neq c'} \frac{|\mathcal{U}_c| |\mathcal{U}_{c'}|}{m(m-1)} \widehat{\MMD}^2_{\mathcal{H}} \big( \widehat{\mb{p}}^l(\mathcal{U}_c), \widehat{\mb{p}}^l(\mathcal{U}_{c'}) \big),
\end{align}
where $\widehat{\mb p}^l( \mathcal{U}_c) = ( \widehat{\mb p}^l(\bm{X}^u), \mb{X}^u \in \mathcal{U}_c)$.



\section{The proposed method}

\bibliographystyle{unsrtnat}
\bibliography{references}  %%% Uncomment this line and comment out the ``thebibliography'' section below to use the external .bib file (using bibtex) .


%%% Uncomment this section and comment out the \bibliography{references} line above to use inline references.
% \begin{thebibliography}{1}

% 	\bibitem{kour2014real}
% 	George Kour and Raid Saabne.
% 	\newblock Real-time segmentation of on-line handwritten arabic script.
% 	\newblock In {\em Frontiers in Handwriting Recognition (ICFHR), 2014 14th
% 			International Conference on}, pages 417--422. IEEE, 2014.

% 	\bibitem{kour2014fast}
% 	George Kour and Raid Saabne.
% 	\newblock Fast classification of handwritten on-line arabic characters.
% 	\newblock In {\em Soft Computing and Pattern Recognition (SoCPaR), 2014 6th
% 			International Conference of}, pages 312--318. IEEE, 2014.

% 	\bibitem{hadash2018estimate}
% 	Guy Hadash, Einat Kermany, Boaz Carmeli, Ofer Lavi, George Kour, and Alon
% 	Jacovi.
% 	\newblock Estimate and replace: A novel approach to integrating deep neural
% 	networks with existing applications.
% 	\newblock {\em arXiv preprint arXiv:1804.09028}, 2018.

% \end{thebibliography}




==> sections/benchmark.tex <==
\section{benchmark}
\subsection{Measuring the Performance Impact of Semantic Similarity}

As described in \autoref{sec:preliminary}, the semantic similarity between the labeled and the unlabeled data is key to the performance of \ac{ncd}. However, the benchmarks used in previous work do not consider this issue, and mostly focus on the number of labeled and unlabeled classes as the indicator of difficulty. To systematically measure the impact the similarity has on \ac{ncd} performance, we propose two new benchmarks that contain different combinations of labeled sets and unlabeled sets of varying semantic similarity.

% Maybe we need a figure here to illustrate the dataset split?
% Numbers as words or numerals?

Our first benchmark in based on CIFAR100 \cite{krizhevsky2009learning}. To split the data into groups of similar classes, we leverage the hierarchy of the dataset, which consists of twenty superclasses, with five subclasses each. We first divide the data into two halves, each consisting of ten superclasses. Then, we split the subsets into a labeled and an unlabeled set, by assigning four subclasses of each superclass to the labeled set and the remaining class to the unlabeled set. In total, we now have two labeled subsets l1 and l2 and two unlabeled subsets u1 and u2, where l1 is closely related to u1 and l2 is closely related to u2. Additionally, we define a third labeled set l3, that contains half of the superclasses in l1 and half of the superclasses in l2. Under our assumptions it would be expected that combining u1 and l1 delivers better performance than the combining it with l2, with l3 somewhere in between. Thus, combining different splits of labeled and unlabeled classes allows us to investigate the impact semantic similarity has on \ac{ncd} performance.

While this benchmark allows us to empirically prove our theory, it is based on a rather small dataset, and our approach of splitting the data into subsets essentially halves the amount of data the models are trained on. To also conduct our experiments in a more realistic setting, we propose a second benchmark based on the much larger ImageNet dataset \cite{deng2009imagenet}. While the ImageNet labels are based on the WordNet hierarchy \cite{miller1995wordnet}, this hierarchy is impractical as outlined by \citeauthor{santurkar2020breeds} in \cite{santurkar2020breeds}. The reasons include the heavily imbalanced number of subclasses per superclass, the often very abstract nature of some superclasses, and the possibility of one subclasse having multiple superclasses. To address these issues, \citeauthor{santurkar2020breeds} proposed an altered hierarchy as well as several ImageNet subsets based on it. One of them is the Entity30 benchmark, which consists of 240 ImageNet classes divided into 30 superclasses with 8 subclasses each. Based on Entity30, we split the data into three labeled and two unlabeled set similar to our first benchmark.

==> sections/metrics.tex <==
\subsection{Information leakage in NCD}
\label{sec:preliminary}

In this section, we introduce a formal framework of the novel class discovery (NCD). To proceed, let $(\mb{X}^l, Y^l)$ and $(\mb{X}^u, Y^u)$ be random samples under the \emph{labeled/unlabeled probability measures} $\mathbb{P}^l$ and $\mathbb{P}^u$, respectively.
Here $\mb{X}^l \in \mathcal{X}^l \subset \mathbb{R}^d$ and $\mb{X}^u \in \mathcal{X}^u \subset \mathbb{R}^d$ are the labeled/unlabeled feature vectors. $Y^l \in \mathcal{C}^l$ and $Y^u \in \mathcal{C}^u$ are the labels of labeled/unlabeled data, where $\mathcal{C}^l / \mathcal{C}^u$ is the label set under the labeled probability measure $\mathbb{P}^l / \mathbb{P}^u$.
There are labeled dataset $\mathcal{L}_n = (\mb{X}_i^{l}, Y_i^{l})_{i=1, \cdots, n}$ independently drawn from the labeled probability measure $\mathbb{P}^{l}$, and unlabeled dataset $ \mathcal{U}_m = (\mb{X}_i^{u})_{i=1, \cdot, m}$ independently drawn from the unlabeled probability measure $\mathbb{P}_{\mb{X}}^u$. \textbf{Our primary goal is to make prediction to $Y^u_i$ under the probability measure $\mathbb{P}^{u}$ given $\mb{X}_i^{u}$.} We now give a general definition of NCD.

\begin{definition}[Novel class discovery]
	Given a labeled probability measure $\mathbb{P}^l$ on $\mathcal{X}^l \times \mathcal{C}^l$, an unlabeled probability measure $\mathbb{P}^u$ on $\mathcal{X}^u \times \mathcal{C}^u$, and a labeled dataset $\mathcal{L}_n$ and an unlabeled dataset $\mathcal{U}_m$, novel class discovery aims to predict the labels of the unlabeled dataset based on $\mathcal{L}_n$ and $\mathcal{U}_m$, where $\mathcal{C}^u \neq \mathcal{C}^l$.
\end{definition}

\sout{In general, NCD is a subgroup of transfer learning, with both domains and tasks are different. Yet, it has own distinct characteristics in the existence of new classes on the unlabeled dataset.} In Figure \ref{fig:compare}, we summarize the relationship/different among three major learning paradigms (with both labeled and unlabeled datasets): NCD, semi-supervised learning and transfer learning.

% Then, the training samples $\mathcal{D}_\old = (\mb{X}_{\old,i}, Y_{\old,i})^{n_\old}_{i=1}$ are independent and identically drawn from the old probability measure $\mathbb{P}_\old$ on $(\mb{X}_l, Y_l)$. Note that $\mathcal{C}^{(l)}$ may not be fully observed by $\mathcal{D}_\old$, thus we denote $\mathcal{C}^{\text{sub}}_{\old} = \text{set}\{ (Y_i)_{i=1}^n \}$ to clarify. 
% For the new distribution, we observe $n_\new$ independent and identically distributed unlabeled data $( \mb{X}_{\new, l})_{l=1}^m$. The new class with respect to the training sample $\mathcal{D}_\old$ is defined as $\mathcal{C}^u / \mathcal{C}^{\text{sub}}_{\old}$.
\red{add more about the marginal information, and $\mathbb{P}_{Y|\mb{X}}$ only.}

Note that it is critical to measure the similarity between $\mathbb{P}^l$ and $\mathbb{P}^u$. As indicated in Figure \ref{fig:compare}, NCD degenerates to the classical SSL when $\mathbb{P}^l = \mathbb{P}^u$, or the transductive transfer learning if $\mathbb{P}_{Y|\mb{X}}^l = \mathbb{P}_{Y|\mb{X}}^u$. 
\sout{Moreover, in practice, there are many pairs of labeled and unlabeled dataset to choose from. For example, fixing the unlabeled dataset as CIFAR-100, we can use CIFAR-10, CIFAR-50 or Image-NET as the labeled dataset. }
Certainly, different pairs of labeled/unlabeled datasets yield various predictive performance. This leads to the following questions: 
\begin{itemize}
	\item How can we tell the self \textit{difficulty} of NCD under $\mathbb{P}^u$ based on unlabeled dataset $\mathcal{U}_m$?
	\item How much does the labeled dataset $\mathcal{L}_n$ under $\mathbb{P}^l$ can help to predict the label under $\mathbb{P}^u$?
\end{itemize}
 To address the questions, we propose the concept of \textit{leakage} to measure the difficulty of NCD. Specifically, the first question concerns the self difficulty of NCD under an unsupervised manner, which predicts labels solely based on marginal information of $\mb{X}^{u}$, is highly related to the discriminative information leaked in the marginal distribution, namely \textit{self leakage}. For the second question, we introduce \textit{transfer leakage} to quantify the discriminative information in $\mathbb{P}^u$ leaked in $\mathbb{P}^l$, that is, how much information we can leverage from the labeled dataset to help improve the performance of the unlabeled dataset.

It is worth to point out that investigation of the questions not only can help us to construct benchmark dataset for fair numerical comparison of existing methods (see Section \red{???}), but also inspire our proposed method yielding state-of-the-art performance in NCD (see Section \red{???}).

\subsubsection{Overall leakage}
\red{Change to IPM to make it more general.}
To quantify the \emph{overall leakage} under the probability measure $\mathbb{P}^u$, we turn to measure the discrepancy of $\mb{X}^{u}$ given different labels $Y^u = c; (c \in \mathcal{C}^{u})$. For instance, given two labels $c, c' \in \mathcal{C}^u$, if there exists a transformation $h(\cdot)$ such that the distributions of $h(\mb{X}^u) | Y^u = c$ and $h(\mb{X}^u) | Y^u = c'$ are easily separable (or distance is large), then it is potential feasible to discriminate $c$ and $c'$ under an unsupervised manner. To this end, we introduce Maximum Mean Discrepancy (MMD; \citep{gretton2012kernel}) or Wasserstein-1 distance (\cite{pmlr-v70-arjovsky17a}) to quality the discrepancy of two distributions:
\begin{align}
	\label{def:mmd}
	\MMD_\mathcal{H} \big( \mathbb{P}^u_{\mb{X}^u | Y^u=c'}, \mathbb{P}^u_{\mb{X}^u | Y^u = c} \big) := \sup_{h \in \mathcal{H}} \Big( \mathbb{E}\big( h( \mb{X}^u) \mid Y^u = c \big) - \mathbb{E}\big( h( \mb{X}^u) \mid Y^u = c'\big) \Big)
\end{align}
where $\mathcal{H}$ is a class of functions $h: \mathcal{X}^u \to \mathbb{R}$, which is usually specified as the unit ball in a reproducing kernel Hilbert Space (RKHS), or a deep neural network as in W-GAN \citep{pmlr-v70-arjovsky17a}.
From \eqref{def:mmd}, when $\MMD$ is large, it provides a relatively large possibility to find a good transformation on $\mb{X}^u$ discriminating labels in an unsupervised manner. 

% \noindent \textbf{Remark.} In \eqref{def:mmd}, we use a generative model $\mathbb{Q}_{\mb{X}^u | Y^u=c}$ to quantify the overall leakage, one may suggest using a discriminative model $\mathbb{Q}( Y^u = c| \mb{X}^u ); (c \in \mathcal{C}^u)$ to quality the leakage of the prediction under $\mathbb{Q}$. It is sensible in supervised learning, when $(\mb{X}^u, Y^u)$ is observed in training set. In our case, our goal to measure the leakage based on an unsupervised manner, where the discrepancy of $\mathbb{Q}_{\mb{X}^u | Y^u=c}$ is more reasonable.

For multi-class discrepancy, we mimic the one-vs-rest nature by taking the minimum discrepancy over all rest classes, which takes the discrepancy to the closest class. Taken together, the overall leakage is defined as follows.
\begin{definition}[Self leakage]
	\label{def:S-leak}
	The self \textit{leakage} of NCD prediction on $\mathbb{P}^u$ is defined as 
	\begin{equation}
	\text{S-Leak}( \mathbb{P}^u ) = \mathbb{E} \Big( \MMD^2 \big( \mathbb{P}^u_{\mb{X}^u | Y^u }, \mathbb{P}^u_{\widetilde{\mb{X}}^u | \widetilde{Y}^u } \big) \Big),
	\end{equation}
	where $(\mb{X}^u, Y^u), (\widetilde{\mb{X}}^u, \widetilde{Y}^u) \sim \mathbb{P}^u$ are independent copies under $\mathbb{P}^u$, and the expectation is taken with respect to $Y^u$ and $\widetilde{Y}^u$. 
\end{definition}

\begin{lemma}
	\label{lemma:ol-zero}
	$\text{O-Leak}( \mathbb{P}^u ) = 0$ if and only if $Y^u$ is independent with $\mb{X}^u$, that is, for any $c \in \mathcal{C}^u$:
	$$
	\mathbb{P}^u( Y^u = c \mid \mb{X}^u ) = \mathbb{P}^u(Y^u = c).
	$$
\end{lemma}
Lemma \ref{lemma:ol-zero} indicates that if there is no overall leakage on $\mb{X}^u$ when predicting $Y^u$, then the best way to predict $Y^u$ given $\mb{X}^u$ is majority voting on $Y^u$. In practice, NCD dataset are often pre-balanced, that is, $\mathbb{P}^u(Y^u = c) = 1/|\mathcal{C}^u|$ for all $c \in \mathcal{C}^u$. 
% Then, \eqref{eqn:ol_gen_model} can be replaced as $\mathbb{P}^u(Y^u=c|\mb{X}^u) = \mathbb{P}(Y^u = c' | \mb{X}^u)$, and the best prediction is random guess. 
Therefore, the proposed overall leakage is a reasonable criterion to measure the predictive information leakage on $\mb{X}^u$, and the overall difficulty of NCD.


Suppose the labels $(Y^u_i)_{i=1, \cdot, m}$ for the unlabeled dataset are observed, denote $\mathcal{U}_c = \{ \mb{X}^u_i \in \mathcal{U}_m: Y_i^u = c\}$ as the sub-sample set under label $c$, the \textit{overall leakage} is empirically evaluated as 
\begin{align}
	\label{eqn:emp_overall_leak}
	\widehat{\text{O-Leak}}( \mathbb{P}^u ) & = \frac{2}{m(m-1)} \sum_{1 \leq i < i' \leq m} \widehat{\MMD}^2_{\mathcal{H}} \big( \mathcal{U}_{Y_i^u}, \mathcal{U}_{Y^u_{i'}} \big) \\
	& = \sum_{c, c' \in \mathcal{C}^u; c \neq c'} \frac{|\mathcal{U}_c||\mathcal{U}_{c'}|}{m(m-1)} \widehat{\MMD}^2_{\mathcal{H}} \big( \mathcal{U}_c, \mathcal{U}_{c'} \big),
\end{align}
where $\widehat{\MMD}_{\mathcal{H}}$ is an empirical evaluation of MMD based on $\mathcal{H}$. For example, 
letting $\mathcal{H} = \mathcal{H}_K$ as a RKHS, we have
\begin{align}
	\label{eqn:emp_mmd}
	\widehat{\MMD}^2_{\mathcal{H}} ( \mathcal{U}_{c}, \mathcal{U}_{c'}) & = \frac{1}{|\mathcal{U}_{c}| \big( |\mathcal{U}_{c}| - 1 \big)} \sum_{ \mb{X}, \mb{X}' \in \mathcal{U}_{c}; \mb{X} \neq \mb{X}'} k( \mb{X}, \mb{X}' ) \\
	& + \frac{1}{|\mathcal{U}_{c'}| \big( |\mathcal{U}_{c'}| - 1 \big)} \sum_{ \mb{X}, \mb{X}' \in \mathcal{U}_{c'}; \mb{X} \neq \mb{X}'} k( \mb{X}, \mb{X}' ) \nonumber \\ 
	& = \quad - \frac{1}{|\mathcal{U}_{c}| |\mathcal{U}_{c'}| } \sum_{ \mb{X} \in \mathcal{U}_{c} } \sum_{ \mb{X}' \in \mathcal{U}_{c'}} k( \mb{X}, \mb{X}'),
\end{align}
where $k(\cdot, \cdot)$ is a reproducing kernel, such as Gaussian kernel. Note that a large $\widehat{\text{O-Leak}}_m(\mathbb{P}^u )$ implies that there is clear discrepancy on $\mb{X}^u$ among different classes, which indicates potential capability of unsupervised learning with $\mb{X}^u$ predicting its label. In practice, $\mb{X}^u$ is usually replaced by a latent feature from representation learning.

\subsubsection{Transfer leakage}
For unsupervised learning, it is usually quite difficult to learn such as good transformation solely based on $\mb{X}^u$. Instead, NCD takes account of the conditional probability $\mathbb{P}^l_{Y | \mb{X} }$ (usually presented by a pre-trained neural network) from a labeled dataset to help construct a transformation. Thus, we consider \emph{transfer leakage} of $\mathbb{P}^l$ on $\mathbb{P}^u$.

The main idea is to quantify the discrepancy of $\mathbb{P}^l_{Y|\mb{X}}$ on $\mb{X}^u$ under the new measure $\mathbb{P}^u$. Then, \emph{transfer leakage} can be defined as follows.

\begin{definition}[Transfer leakage]
	\label{def:T-leak}
	The transfer leakage of NCD prediction under $\mathbb{P}^u$ based on the labeled conditional probability $\mathbb{P}^l_{Y^l|\mb{X}^l}$ is 
	\begin{equation}
	\text{T-Leak}( \mathbb{P}^u, \mathbb{P}^l ) = \mathbb{E} \Big( \MMD^2 \big( \mathbb{P}^u_{ \mb{p}^l(\mb{X}) | Y }, \mathbb{P}^u_{\mb{p}^l(\mb{X}') \mid Y'} \big) \Big),
	\end{equation}
	where $(\mb{X}, Y), (\mb{X}', Y) \sim \mathbb{P}^u$ are independent copies, the expectation is taken with respect to $Y$ and $Y'$ under $\mathbb{P}^u$, and $\mb{p}^l(\mb{X}^u)$ is the conditional probability under $\mathbb{P}^l_{Y|\mb{X}}$ on an unlabeled instance $\mb{X}^u$, which is defined as
	$$
	\mb{p}^l(\mb{x}) = \big(\mathbb{P}^l\big( Y^l=c \mid \mb{X}^l = \mb{x} \big) \big)_{c \in \mathcal{C}^l}.
	$$
\end{definition}
With the similar manner in Definition \ref{def:O-leak}, the definition of transfer leakage is to measure the discrepancy of $\mb{p}(\mb{X}^u)$ under different new classes of $\mathbb{P}^u$, which indicates the  informative leakage of $\mathbb{P}^u$ on $\mathbb{P}^l$, and potential capability of transferring information from $\mathbb{P}^l$ to $\mathbb{P}^u$.

\begin{lemma}
	\label{lemma:tl-zero}
	$\text{T-Leak}( \mathbb{P}^u, \mathbb{P}^l ) = 0$ if and only if $Y^u$ is independent with $\mb{p}^l(\mb{X}^u)$, that is, for any $c \in \mathcal{C}^u$:
	\begin{equation}
		\label{eqn:tl-indep}
		\mathbb{P}^u\big( Y^u = c \mid \mb{p}^l(\mb{X}^u) \big) = \mathbb{P}^u(Y^u = c).
	\end{equation}
	Moreover, if $ \mathbb{P}^u = \mathbb{P}^l$, then \eqref{eqn:tl-indep} can be replaced as:
	$$
	\mathbb{P}^l\big( Y^l = c \mid \mb{X}^l \big) = \mathbb{P}^l(Y^l = c).
	$$
\end{lemma}

Given an estimated conditional probability $\widehat{\mathbb{P}}^l_{Y^l|\mb{X}^l}$, usually presented as a pre-trained neural network, we evaluate $\mb{X}^u$ on $\widehat{\mathbb{P}}^l_{Y^l|\mb{X}^l}$ as $\widehat{\mb p}^l(\mb{X}^u) = \big(\widehat{\mathbb{P}}^l\big( Y^l=c | \mb{X}^l = \mb{X}^u \big) \big)_{c \in \mathcal{C}^u}$, then the empirical transfer leakage is computed as
\begin{align}
	\label{eqn:emp_overall_leak}
	\widehat{\text{T-Leak}}( \mathbb{P}^u, \mathbb{P}^l ) & = \frac{2}{m(m-1)} \sum_{1\leq i< i' \leq m}  \widehat{\MMD}^2_{\mathcal{H}} \big( \widehat{\mb p}^l( \mathcal{U}_{Y_i^u} ),  \widehat{\mb p}^l( \mathcal{U}_{ Y^u_{i'} } ) \big) \nonumber \\
	& = \sum_{c, c' \in \mathcal{C}^u; c \neq c'} \frac{|\mathcal{U}_c| |\mathcal{U}_{c'}|}{m(m-1)} \widehat{\MMD}^2_{\mathcal{H}} \big( \widehat{\mb{p}}^l(\mathcal{U}_c), \widehat{\mb{p}}^l(\mathcal{U}_{c'}) \big),
\end{align}
where $\widehat{\mb p}^l( \mathcal{U}_c) = ( \widehat{\mb p}^l(\bm{X}^u), \mb{X}^u \in \mathcal{U}_c)$.



